JanusAQP: Efficient Partition Tree Maintenance for Dynamic Approximate Query Processing

Approximate query processing over dynamic databases, i.e., under insertions/deletions, has applications ranging from high-frequency trading to internet-of-things analytics. We present JanusAQP, a new dynamic AQP system, which supports SUM, COUNT, AVG, MIN, and MAX queries under insertions and deletions to the dataset. JanusAQP extends static partition tree synopses, which are hierarchical aggregations of datasets, into the dynamic setting. This paper contributes new methods for: (1) efficient initialization of the data synopsis in the presence of incoming data, (2) maintenance of the data synopsis under insertions/deletions, and (3) re-optimization of the partitioning to reduce the approximation error. JanusAQP reduces the error of a state-of-the-art baseline by more than 60% using only 10% storage cost. JanusAQP can process more than 100K updates per second in a single node setting and keep the query latency at a millisecond level.

==> DynamicPASS_ICDE FULLARXIV/abstract.tex <==
\begin{abstract}
Approximate query processing over dynamic databases, i.e., under insertions/deletions, has applications ranging from high-frequency trading to internet-of-things analytics.
We present \sys, a new dynamic AQP system, which supports SUM, COUNT, AVG, MIN, and MAX queries under insertions and deletions to the dataset. 
\sys extends static partition tree synopses, which are hierarchical aggregations of datasets, into the dynamic setting.
This paper contributes new methods for: (1) efficient initialization of the data synopsis in the presence of incoming data, (2) maintenance of the data synopsis under insertions/deletions, and (3) re-optimization of the partitioning to reduce the approximation error. 
\sys reduces the error of a state-of-the-art baseline by more than 60\% using only 10\% storage cost. \sys can process more than 100K updates per second in a single node setting and keep the query latency at a millisecond level.

% \xl{60\% is a bit conservative and i use it because sometimes even RS outperforms DeepDB, and 60\% is an improvement that also applied to RS. We can have even better accuracy like we had in static pass by using additional samples that can work with data skipping. Data skipping in current experiment improves query latency only.}

\end{abstract}

==> DynamicPASS_ICDE FULLARXIV/additionals.tex <==

In this section we propose new algorithms for constructing a partition over the samples items $\samples$. Our algorithms can be used in different scenarios: i) construct a partition the first time over $\samples$, ii) construct a new partition if the re-partition is needed after a number of updates in our dataset, and iii) check if repartition is needed after an insertion or deletion of an item, i.e., is there a partition with significantly less error than the current partition?
%In the end of this section we formally describe how Dynamic PASS decides when a re-partition/re-construction of $\PASStree$ is needed.

In~\cite{liang2021combining} the authors proposed algorithms for constructing near optimal partitions.
However, most their algorithms run in time roughly $O(km\log m)$. For the offline version of the problem their algorithm is very efficient since it is linear in both parameters $k, m$. Ideally, in the dynamic setting, we do not want the update procedure to depend linearly on $m$, i.e., the number of samples we store. Here we design data structures and algorithms that run the re-partition (or the check if there is a better partition) in only $O(k)$ time, ignoring $\polylog$ factors, which is near-optimal since we have $k$ buckets.

In order to achieve faster algorithms we propose new dynamic data structures for various sub-problems. Mainly, we propose an efficient dynamic data structures such that given a query rectangle, it returns (approximately) the maximum variance of a query completely inside the query rectangle. Using this data structure, we can achieve a very fast construction of $\PASStree$ in any dimension $d$.
For $d=1$ we manage to design a very efficient algorithm making an assumption on the aggregation values of the items. In particular we assume that the values of items are bounded by a polynomial on $N$, i.e. the total number of items in the full dataset. This is usually the case in real datasets so it is not a strong assumption and it is made in several papers~\cite{guha2006approximation} for constructing histograms with low error. %We notice that the assumption is not needed in higher dimensions.

We start by introducing some basic notation and by defining some basic notions. Then we describe our new dynamic data structures for finding maximum error queries.
We continue by presenting the partition algorithm for $d=1$ and the partition algorithm for any dimension $d>1$.
In the end of this section we show an algorithm to decide when re-partition is needed.


\subsection{Preliminaries}
The goal of \sys is to construct a dynamic partition tree $\PASStree$ such that the maximum error (confidence interval) of a query is minimized. Recall that the leaf nodes of $\PASStree$ define a partition over the samples $\samples$.
As we discussed in previous sections the number of samples $H$ (catch-up phase) is going to be much larger than the number of samples in $\samples$. In particular, the sampling rate of $H$ in the end of the catch-up phase is significantly higher than the sampling rate of $\samples$ we store in $\PASStree$. Hence we expect that the error (variance) of nodes in $U_2$ will be much lower comparing to the error of the nodes in $U_1$ for a query $q$. So we focus on finding a partition that minimizes the longest confidence interval of any possible query considering only the error from the leaf nodes that partially intersect the query.

As shown in~\cite{liang2021combining}, in order to find the query with the worst confidence interval in the partition defined by the leaf nodes of $\PASStree$, it is sufficient to consider only queries that lie completely inside the leaf nodes of $\PASStree$.
Indeed by considering only these queries we can still get a $\sqrt{k}$-approximation for COUNT and SUM queries over the optimum partition considering all queries. The approximation factor improves to $\sqrt{2}$ for $d=1$. For AVG queries the error of the optimum partition considering queries completely inside the leaf nodes is the same with the maximum error considering every possible query. So without loss of generality we solve the optimization problem of finding a partition that minimizes the maximum error considering only queries that lie completely inside the buckets of a partition.


%Static PASS~\cite{hellerstein2008quantitative} tries to find a tree structure such that its leaf nodes define a partition over the samples $\samples$ to (approximately) minimize the length of the longest confidence interval. Equivalently, in PASS they are trying to find a partition that minimizes the maximum error. The authors in~\cite{liang2021combining} argue that instead of looking over all possible queries to minimize the maximum error they focus on queries that lie completely inside one bucket. Indeed, the optimum partition considering only queries that lie completely inside a bucket has error at most $\sqrt{k}$ times more than the error over the optimum partition for COUNT/SUM queries. For AVG queries the error of the optimum partition considering queries completely inside buckets is the same with the maximum error considering every possible query.


%Similarly to~\cite{liang2021combining}, considering only queries completely inside a bucket gives a $\sqrt{k}$ approximation for COUNT/SUM queries and $1$-approximation (optimum) for AVG queries. For $1$D it gives a $\sqrt{2}$ approximation for COUNT/SUM queries.

Let $u$ be a leaf node of $\PASStree$ and let $q$ be a query completely inside $R_u$. In this case notice that $w_u=1$ for all types of queries.
From Section~\ref{sec:estimators}, recall that the variance of any COUNT or SUM query completely inside $R_u$ has a factor $\frac{N_u^2}{m_u^2}$. This factor is the same in all queries inside $u$ so without loss of generality we can skip it from the variance definition (considering queries inside $R_u$).
Furthermore, notice that the confidence interval of any query inside $R_u$ has a factor $\frac{1}{m_u}$ which is also the same. Hence, the problem of finding the query with the largest confidence interval in $u$ is equivalent with the problem of finding the query $q$ in $u$ that maximizes the following function.
If $q$ is a COUNT or SUM query:
$$\nu_s(q)=m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2,$$
and if $q$ is an AVG query:
$$\nu_s(q)=\frac{1}{|q|^2}\left[m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2\right].$$


In order to make sure that we return accurate estimators we require that each bucket contains a sufficiently large amount of samples, roughly $\Omega(\frac{1}{\alpha}\log m)$ samples, where $\alpha$ is the sampling rate of $\samples$.
%If that holds, it is known from~\cite{liang2021combining} that with high probability the ratio $\frac{N_u}{m_u}$ for any possible leaf node $u$ will be within a constant factor from the ratio $N/m$, so it will be almost the same for any bucket we construct.
Furthermore, we study queries that contain at least $\delta m$ samples from each bucket that they partially intersect, for a small parameter $\delta<1$. Otherwise a query does not include many samples and we are not be able to return an accurate estimator along with a provable confidence interval. We note that these assumptions were also made in~\cite{liang2020fast}.
%Finally, we define the following notation which is useful in the next subsections. For a rectangle $R$, let $\optVar(R)$ be the variance of the query with the maximum variance in $R$.

==> DynamicPASS_ICDE FULLARXIV/background.tex <==
\section{Background}
We first introduce the core concepts behind the synopses used in this work. 

\subsection{Dynamic Approximate Query Processing}
We assume an initial database table $\fullData^{(0)}$.
This table $\fullData^{(0)}$ is continuously modified through a stream of insertions and deletions of tuples.
As a design principle, we assume that insertions are common but deletions are rare.
With each insertion or deletion operation, the table evolves over time with a new \textbf{state} at each time step $i$:
$\fullData^{(0)},\fullData^{(1)},\ldots,\fullData^{(i)}, \fullData^{(i+1)},\ldots$
A \textbf{synopsis} is a data structure that summarizes the evolving table. 
For each $\fullData^{(i)}$, there is a corresponding synopsis $\Sigma^{(i)}$:
$\Sigma^{(0)},\Sigma^{(1)},\ldots,\Sigma^{(i)}, \Sigma^{(i+1)},\ldots$

In DAQP, the problem is to answer queries as best as possible from only the $\Sigma^{(i)}$.
For a query $q$, the estimation error is defined as the difference between the estimated result (using the synopsis) and the true result (using the current database state): 
\[ \textsf{Error}(q, \Sigma^{(i)}) = |q(\fullData^{(i)}) ~~ -  ~~ q(\Sigma^{(i)})|\]
We further assume that there is sufficient cold/archival storage to store the current state of the table $\fullData^{(i)}$.
This data can be accessed in an offline way for initialization, re-optimization, and logging purposes but not for query processing.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/teaser.png}
    % Xi: 0.8 => 1 to make the text more readable.
    \caption{The core data structure in \sys is based on the PASS data structure~\cite{liang2021combining} that summarizes a dataset with a tree of aggregates at different levels of resolution (granularity of partitioning). Associated with the leaf nodes are stratified samples. The two stage synopsis structure can be optimally partitioned to minimize error.  \label{fig:teaser}}
\end{figure}

There are a few notable differences from the ``streaming'' setting. First, most data streaming models do not support arbitrary record deletion, i.e., as studied in~\cite{poepselland}. We find that in many use-cases limited support for deletion is needed due to records that are invalidated through an out-of-band, asynchronous data process like fraud detection or financial auditing. Next, most streaming settings enforce a single pass over the data with limited overall memory. We do not make this assumption and allow for archival storage and slow access to old data. This is a more realistic AQP setting where all data are stored, however, there is limited working memory for a fast, approximate query answering service. 

\subsection{Related work}
There is significant research in histograms and their variants that is highly relevant to this project~\cite{jagadish1998optimal, koudas2000optimal, jagadish2001global}.
V-Optimal histograms construct buckets to minimize the cumulative variance~\cite{jagadish1998optimal}. There are works on
multi-dimensional histograms~\cite{lazaridis2001progressive}, and histograms on the streaming/dynamic setting~\cite{guha2006approximation, gilbert2002fast}.
Like histograms, \sys constructs partitions over attribute domains and aggregates within the partition. However, we contribute different partition optimization criteria than typically used in histograms and novel techniques based on geometric data structures to scale partitioning into higher dimensions. Furthermore, our system works in the general dynamic setting, unlike~\cite{gilbert2002fast} where the number of total items must remain the same.
Another related area of research is into mergeable summaries that compute a partition of the data and optimize sampling at a data partition level~\cite{rong2020approximate, liang2020fast, agarwal2012mergeable, gan2020coopstore, poepselland}. \reviewtwo{The \syn used in \sys very much behaves like a mergeable summary but it combines low-error statistics over pre-computed partitioning of the space, along with stratified sampling to improve the error over comparing to traditional mergeable summaries for aggregation queries.}
Furthermore, some prior work mostly focuses on a streaming setting without support for deletion~\cite{poepselland}.
Similarly, sketches~\cite{cormode2011sketch, cormode2011synopses} have been used to find a summary of data to answer approximately a variety of queries efficiently. However, they also do not handle arbitrary range queries using space independent of the size of the full database. Mergeable summaries and sketches usually focus on optimizing different types of problems such that frequency queries, percentile queries, etc.
This paper shows how to operationalize a general DAQP system for aggregation queries with both systems and algorithmic contributions relating to the design of dynamic synopses and their continuous optimization. Our system can handle arbitrary updates and can estimate any arbitrary predicate query with provable confidence intervals.

In databases, a number of tree-based indexes, such as the improved $R^*$ tree~\cite{jurgens1998r}, have been used to support range aggregation queries efficiently.
The space of such indexes is (super-)linear with respect to the input items.
The query procedures need to have access to the entire tree-index that contains the entire dataset. That leads to high communication throughput or high I/O operations comparing to \sys where the queries are executed in a small synopsis of data stored in a local machine or RAM with zero communication throughput.
%The space of such indexes is super-linear with respect to the input items so they cannot be used for high volume of data, which is the main focus in this paper.
In another line of work, tree-based data structured are used to return a set of $k$ uniform samples in a query range. More specifically, in~\cite{joshi2008materialized, wang2015spatial} the authors construct indexes such that given a query range $Q$ and a parameter $k$, they return $k$ uniform samples from the input items that lie inside $Q$. These samples can be used to estimate any aggregation query in the range query $Q$.
There are several issues with these indexes in our setting.
First, the design of the index in~\cite{joshi2008materialized} makes their structure inherently static and it cannot be maintained efficiently.
Furthermore, the estimation error in both indexes is the same as the error in the simple uniform random sampling schema. In Section~\ref{sec:experiments}, we show that the error of our new index in real data sets is always less than half of the error in uniform random sampling, so our new index always outperforms these range sampling indexes.
In addition, the communication throughput or the I/O operations during a query procedure of these indexes is a function of $N$, i.e. the size of the input set, so they cannot be used on big data.
Finally, the dynamic tree structure in~\cite{lazaridis2001progressive} can store a synopsis of data in a tree-based index and use only this synopsis/index to return estimations of a range aggregation queries, which is also the case in our system \sys. However, there are two main differences. The index in~\cite{lazaridis2001progressive} returns a good estimation only if an assumption about the spatial/value-domain distribution of the data is made, while \sys uses stratified sampling and it always returns unbiased estimators with small error without assuming any distribution over the data. Furthermore, while their partition tree in~\cite{lazaridis2001progressive} can handle dynamic updates, its structure/partitioning remains unchanged. In our index we maintain a near-optimal partitioning over the updates. As we show in Section~\ref{sec:exp-del}, running experiments on real data, re-partitioning is essential in order to maintain a small error.

Dynamic AQP problems have been discussed in prior work~\cite{garofalakis2001approximate}, however, most existing systems have focused on a static data warehousing setting~\cite{agarwal2013blinkdb}. The Aqua system~\cite{acharya1999aqua} did consider the maintenance of its synopsis data structures under updates. However, these synopses were relatively simple and only samples and histograms. Furthermore, we discuss systems issues such as catch-up processing that was not discussed in~\cite{acharya1999aqua} or any subsequent work~\cite{gibbons2002fast}.  

Many new AQP techniques use machine learning.
The basic ideas exist for a while, e.g., ~\cite{jermaine2003robust,jin2006new}. Recently, there are more comprehensive solutions that train from a past query workload~\cite{park2017database} or directly build a probabilistic model of the entire database~\cite{hilprecht2019deepdb, yang2019deep}.
We show that these systems are not optimized for a dynamic setting. Even when they can be updated efficiently with warm-start training, their throughput is much lower than \sys.

\subsection{Partition Trees for AQP}
\label{sec:partTreeAQP}
We propose a new dynamic data synopsis and optimization strategy that is an extension of our previous work~\cite{liang2021combining}. In particular, we proposed a system called PASS (which we call \prior for ``static partition tree''). 
\prior synopses are related to works such as~\cite{lazaridis2001progressive} in the data cube literature and hybrid AQP techniques~\cite{peng2018aqp++}.
We showed that with appropriate optimization of the partitioning conditions, an \prior could achieve state-of-the-art accuracy in AQP problems.

\subsubsection{Construction}
An \prior is a synopsis data structure used for answering aggregate queries over relational data.
To use \prior, the user defines an \emph{aggregation column} (numerical attribute to aggregate) and a \emph{set of predicate columns} (columns over which filters will be applied).
An \prior consists of two pieces: (1) a hierarchical aggregation of a dataset, and (2) a uniform sample of data for each of the leaf partitions (effectively a stratified sample over the leaves).
The system returns a synopsis that can answer SUM, COUNT, AVG, MIN, and MAX aggregates over the aggregation column filtered by the predicate columns.
Figure \ref{fig:teaser} illustrates a partition tree synopsis over toy stock-order data.

To understand how this structure is useful, let us overview some of its formal properties.
A \emph{partition} of a dataset $\fullData$ is a decomposition of $\fullData$ into disjoint parts $\fullData_1,...,\fullData_B$.
Each $\fullData_i$ has an associated partitioning condition, a predicate that when applied to the full dataset as a filter retrieves the full partition.
Partitions naturally form a hierarchy and can be further subdivided into even more partitions, which can then be subdivided further.
A \emph{static partition tree} $\PASStree$ is a tree with $B$ nodes (where each node corresponds to a partition) with the following invariants: (1) every child is a subset of its parent, (2) all siblings are disjoint, and (3) the union of all siblings equals the parent.

In an \prior, each node of the tree is associated with SUM, COUNT, MIN, and MAX statistics over the items in $\fullData$ that lie inside the node.
\prior synopses have a flexible height to tradeoff accuracy v.s. storage.
In shorter trees, the leaf nodes of an \prior can cover large subsets of data and vice versa in deeper trees.
Note how each layer of the tree in Figure \ref{fig:teaser} aggregates the lower layer over coarser-and-coarser aggregation conditions (first by ``sector'' and then by ``order type'').

This structure works well when the queries align with partition boundaries. For example, a user aggregating total orders by ``order type'' in Figure \ref{fig:teaser} would get an exact answer with no approximation. The challenge is to answer queries with predicates that partially intersect partitions.
Due to the tree invariants, the set of partial intersections can be fully determined at the leaf nodes.
To estimate the contributions of these partial intersections, an \prior associates a uniform sample of tuples \emph{within that partition} for each leaf node.

\subsubsection{Query Processing}
Using an \prior, a user can estimate the result of a query as follows. Essentially, the query processing algorithm identifies ``fully covered'' nodes that are contained in the query predicate and ``partially covered'' ones that overlap in some way. Exact statistics from the ``fully covered'' nodes can be used, while estimates can be used to determine the contribution of ``partially covered'' ones. We present SUM, COUNT, AVG for brevity, but it is also possible to get estimations for MIN and MAX.

\vspace{0.5em} \noindent  \textbf{Step 1: Frontier Lookup. }  Given a query predicate $q$, traverse the tree top-down to retrieve two sets of nodes partitions: $R_{cover}$ (nodes that fully cover the predicate) and $R_{partial}$ (nodes that partially intersect the predicate). Nodes that do not intersect the predicate can be ignored.

\vspace{0.5em} \noindent \textbf{Step 2: Partial Aggregation } For each partition in $R_{cover}$, we can compute an exact ``partial aggregate'' for the tuples in those partitions. For a SUM/COUNT query $q$: $agg =  \sum_{R_i \in R_{cover}} SUM(R_i)$,
for an AVG query, we weight the average by the relative size of the partition: $agg =  \sum_{R_i \in R_{cover}} SUM(R_i) \frac{N_i}{N_q}$, where $N_i$ is the size of the partition $R_i$, $N_q$ is the total size in all relevant partitions of query $q$, and $SUM(R_i)=\sum_{t\in R_i\cap \fullData}t.a$ is the sum of the aggregation values of all tuples in the partition $R_i$.

 \vspace{0.5em} \noindent \textbf{Step 3: Sample Estimation. } Each partition in $R_{partial}$ is a leaf node with an associated stratified sample. Within each stratified sample, we use standard AQP techniques to estimate that partition's contribution to the final query result~\cite{agarwal2013blinkdb}. For completeness, we include those calculations here. Suppose a partition $R_i$ has a set $\samples_i$ of $m_i$ samples and there are $N_i$ total tuples in $R_i$.
 We can formulate COUNT, SUM, AVG as calculating an average over transformed attributes:
$f(\samples_i)=\frac{1}{m_i}\sum_{t\in \samples_i}\phi_q(t)$,
where $\phi_q(\cdot)$ expresses all the necessary scaling to translate the samples in query $q$ into an average query population. Let $Predicate(t, q)=1$ if tuple $t$ satisfies the predicate of query $q$, and $0$ otherwise, we have
\begin{itemize}
    \item COUNT: $\phi_q(t)=Predicate(t,q)\cdot N_i$
    \item SUM: $\phi_q(t)=Predicate(t,q)\cdot N_i\cdot t.a$
    \item AVG: $\phi_q(t)=Predicate(t,q)\cdot \frac{m_i}{\sum_{t\in \samples_i}Predicate(t,q)}\cdot t.a$
\end{itemize}
We run such a calculation for each partition that is partially covered. These results are combined with a weighted combination like before. For SUM/COUNT queries it is: $samp = \sum_{R_i \in R_{partial}} f(S_i)$. And for AVG queries, it is: $samp = \sum_{R_i \in R_{partial}} f(S_i) \cdot \frac{N_i}{N_q}$. $N_i$ and $N_q$ can be exactly retrieved from the statistics computed for each partition.

\vspace{0.5em} \noindent \textbf{Step 4: Final Estimate. } The results can be found by taking a sum of the two parts: $result = samp + agg.$ For this result estimate, confidence intervals can be calculated using standard stratified sampling formulas.

\vspace{0.25em} \noindent
\textbf{PASS and \sys comparison. }
As we noted, \sys is an extension of PASS in the dynamic setting.  The main differences and novelties of our new system \sys comparing to PASS are the following: i) PASS finds a static partitioning that is not changing after insertions and deletions of items. In \sys we propose algorithms (Subsection 5.4) that automatically check if a re-partitioning is needed after the dynamic updates.  ii) Even if re-partitioning is allowed in PASS, the algorithms we proposed in ~\cite{liang2021combining} do not run efficiently in the dynamic setting. Here we propose dynamic indexes and algorithms with theoretical guarantees that perform much faster than the algorithms in PASS. iii) Even if we use our new dynamic algorithms in PASS, there is no mechanism to compute the exact statistics of the nodes after a re-partitioning happening and there is no mechanism handling the updates as the re-partitioning is executed. \sys can improve the estimators in the nodes of \syn after a re-partitioning, while handling new dynamic updates and new queries. iv) Last but not least, we implement \sys on Apache Kafka, so it can be used by real database systems.

==> DynamicPASS_ICDE FULLARXIV/conclusion.tex <==
\iffalse
\section{Discussion and Conclusion}
Approximate query processing over dynamic databases has applications ranging from high frequency trading to internet-of-things analytics.
We present \sys, a new dynamic AQP system, which supports SUM, COUNT, AVG, MIN, and MAX queries under insertions and deletions to the dataset. 
The initial results are highly promising, and this basic system has many interesting avenues for future work.
We are particularly interested in physically partitioned \syn synopses. This is possible because the leaf nodes of the dynamic partition tree are disjoint and we can further split a tree into two trees which are in charge of different domains. Each DPT can be run in a different node as a standalone service and we can use a router to forward each request to the right tree for processing. We leave the implementation of a \sys cluster as a future work.
\fi

==> DynamicPASS_ICDE FULLARXIV/dpt.tex <==
\section{Dynamic Partition Trees}\label{sec:dpt}
We discuss how Dynamic Partition Trees (\syn) are constructed, how they answer queries, and how they are maintained under updates. Structurally, a \syn is essentially the same data structure as an \prior; however, the way that the partition statistics and samples are represented differ to allow for incremental maintenance. Figure \ref{fig:dpt} summarizes the basic update process. 

\iffalse
\begin{table}
%\small
\caption{Table of basic notation}
\label{Table:Notation}
\centering
 \begin{tabular}{|c|c|} 
 \hline
 $\fullData$ & Full database\\ \hline
 $N$ & $|\fullData|$\\ \hline
 $\samples$ & Set of reservoir samples\\ \hline
 $H$ & Set of catch-up samples\\ \hline
 $R_i$ & Partition/bucket/rectangle\\ \hline
  $|R_i|$ & $|R_i\cap \samples|$\\ \hline
 $N_i$ & $\fullData\cap R_i$\\ \hline
 $\samples_i$ & $\samples\cap R_i$\\ \hline
 $H_i$ & $H\cap R_i$\\ \hline
 $m_i$ & $|\samples_i|$\\ \hline
 $h_i$ & $|H_i|$\\ \hline
 $m$ & $|\samples|$\\ \hline
 $t$ & Tuple in $\fullData$\\ \hline
 $t.a$ & Aggregation value of tuple $t$\\ \hline
 $\PASStree$ & Partition tree in \syn\\ \hline
 %$\optVar(R)$ & Variance of the maximum variance query in $R$\\ \hline
 %$\maxVar(R)$ & Variance of the query returned by our approximation algorithm
\end{tabular}
\end{table}
\fi

\begin{table}[t]
\footnotesize\vspace{-0.5em}
\caption{Table of basic notation}
\centering
 \begin{tabular}{|c|c|c|c|} 
 \hline
 $\fullData$ & Full database & $H_i$ & $H\cap R_i$ \\ \hline
 $N$ & $|\fullData|$ & $m_i$ & $|\samples_i|$ \\ \hline
 $\samples$ & Set of reservoir samples & $h_i$ & $|H_i|$ \\ \hline
 $H$ & Set of catch-up samples & $m$ & $|\samples|$ \\ \hline
 $R_i$ & Partition/bucket/rectangle & $t$ & Tuple in $\fullData$ \\ \hline
  $|R_i|$ & $|R_i\cap \samples|$ & $t.a$ & Aggregation value of tuple $t$ \\ \hline
 $N_i$ & $\fullData\cap R_i$ & 
 $\PASStree$ & Partition tree in \syn \\ \hline
 $\samples_i$ & $\samples\cap R_i$& &\\\hline
\end{tabular}
\label{Table:Notation}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25]{figures/dpt_update.png}
    % Xi 0.14 => 0.2 to make the text more readable
    \caption{The \syn update process for an insertion or deletion. (1) A set of samples is maintained using a reservoir sampling algorithm. (2) The leaf node statistics are incrementally updated. (3) The updated statistics from the leaf node propagate to the parents. (4) Updated statistics from the parents propagate all the way to the root.  \label{fig:dpt}}
\end{figure}

\subsection{Incrementally Maintaining Nodes}
\label{sec:IncrMaintNodes}
Each node defines a partition and contains statistics (the SUM, COUNT, MIN, and MAX aggregates) of the data contained in that partition.
The key challenge is to keep these statistics up-to-date in the presence of insertions and deletions. 
When an insertion or deletion arrives, an entire path of nodes from the leaf to the root will have to be updated.

\vspace{0.5em} \noindent \textbf{\syn Nodes: } First, we discuss how we represent the statistics in a \syn node. Since the SUM and COUNT are easy to incrementally maintain under both insertions and deletions, we simply store a single SUM and COUNT value for each aggregation attribute. The MIN and MAX values are harder to incrementally maintain. To store the MIN and MAX values, we store the top-k and the bottom-k values in a MIN/MAX heap respectively. The top value of these heaps is equal to the MIN and MAX of all the data in the node. 

\vspace{0.5em} \noindent \textbf{Insert New Record: } When a new record is inserted,  we start from the root and we find the leaf node that the record is contained in. Then, we increment the SUM and COUNT statistics accordingly. Finally for MAX/MIN, we push the new aggregation values onto the heap. If the heap exceeds the size limit $k$, then the bottom value on the heap is removed. 

\vspace{0.5em} \noindent \textbf{Delete Existing Record: } When an existing record is deleted, we find the leaf node that the record is contained in. Then we decrement the SUM and COUNT statistics accordingly. Finally for MAX/MIN, if that aggregation value is contained in the heap it is removed from the heap. \reviewone{This might make the heap smaller than $k$.  Repeated deletes from the same node might fully empty the heap. We stop removing values from the heap when there is only one value left. When the heap reaches a single element the MIN/MAX estimates received from the nodes are outer approximations where the estimated value is larger than the MAX and smaller than the MIN.}
\vspace{-1em}
\subsection{Maintaining Stratified Samples}
Next, we describe how to maintain the samples associated with leaf nodes. \reviewtwo{We maintain samples using the \emph{proportional allocation} of stratified sampling. The number of samples in each stratum should be proportional to the size of the stratum over the size of the population.
%Our system can also support Neyman (or optimal) allocation, however the description is more complicated and the experimental results on the datasets we tried were not different. Hence, we focus only on proportional allocation.
We use a modified version of the well-known technique of \emph{reservoir-sampling}~\cite{vitter1985random} under updates~\cite{gibbons2002fast}.
The details of how we implement this are interesting.
Conceptually, each leaf node is associated with a physically disjoint sample of just that partition, i.e., a stratified sample.
Instead of implementing physical strata for the stratified sampling, we implement large enough virtual partitions of a single global sample. 
This global sample can be maintained using a reservoir sampling algorithm and makes it easier to control the overall size of the synopsis under insertions/deletions as well as simplifies concurrency control}.

\vspace{0.5em} \noindent \textbf{Sample Representation: } The \syn maintains a ``pooled'' sample (all the relevant samples in a single data structure). This set of samples has a target size of $2m$ tuples. At the construction time, we choose a set $\samples$ of $2m$ uniform random samples from $\fullData$. The update procedure ensures that there are always between $m\leq |\samples|\leq 2m$ samples. The leaf nodes index into this ``pooled'' sample selecting only the relevant data to their corresponding partitions. \reviewtwo{Since we get a set of uniform samples, if we make sure that our strata are large enough, the number of samples we get in each stratum satisfies the proportional allocation requirements, up to a factor of $2$, with high probability. We formally show it in Appendix~\ref{appndx:proportional}. This is also the case in the next update operations.}

\vspace{0.5em} \noindent \textbf{Insert New Record: } Suppose we insert a new tuple $t$. If $|\samples|<2m$ we add $t$ in $\samples$. If $|\samples|=2m$, we choose $t$ with probability $\frac{|\samples|}{|\fullData|}$. \reviewone{If it is selected then we replace a point from $\samples$, chosen uniformly at random, with $t$.} %\reviewtwo{This procedure also ensures that the proportional allocation in the stratified sampling is maintained (up to a constant factor).}

\vspace{0.5em} \noindent \textbf{Delete Existing Record: } Next, suppose that we delete a tuple $t$ from $\fullData$. If $t\notin \samples$ we do not do anything. If $t\in \samples$ then we check the cardinality of $\samples$. If $|\samples|>m$ then we only remove $t$ from $\samples$. If $|\samples|=m$ then we skip the set $\samples$ and we re-sample $2m$ items from $\fullData$. As shown in~\cite{gibbons2002fast} this procedure always maintain a set of uniform random samples.
\reviewtwo{As shown in Section~\ref{sec:re-partition} we always check if a stratum is under-represented after a number of deletions. If this is the case then we need to re-sample and re-partition.}
Using a simple dynamic search binary tree of space $O(m)$ we can update the samples $\samples$ stored in $\PASStree$ in $O(\text{height}(\PASStree))$ time.
%\reviewtwo{If we delete half of data in $\fullData$ then we re-sample $2m$ items from $\fullData$. In our applications, deletions are rare comparing to the insertions, so this will not happen.}
%Similarly to the insertion, this procedure guarantees that we maintain the proportional allocation of our stratified sampling (up to a constant factor).

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25]{figures/catchup.png}
    \caption{\sys synopses can be re-initialized online using a multi-threaded implementation to minimize unavailability\label{fig:catchup}}
\end{figure}

\subsection{Re-initialization and Catch-Up}\label{sec:catchup}
As we noted before, repeated deletes on the same leaf partition can degrade the accuracy of the synopsis. As we will see in the next section, it is also possible for repeated insertions to degrade the accuracy as well. In such cases, re-initialization of the \syn may be needed where the data structure is re-built and re-optimized over existing data. 

Enabling periodic re-initialization is crucial for reliable long-term deployment but is challenging because new data will not simply stop arriving during the re-initialization period.
%As the dataset size grows, the amount of time needed for re-initialization will grow as well.
We employ a multi-threaded approach to minimize any period unavailability for processing new data arrival as well as new queries (Figure \ref{fig:catchup}).  When re-initialization is triggered, the main processing thread initiates the construction of a new \syn synopsis
%(the algorithm for determining the optimal partitions is in the next section),
and the following steps are performed:
\vspace{-0.5em}
\begin{enumerate}
	\item Optimization Phase (In Parallel)
	\begin{itemize}
\item The partition optimization algorithm analyzes the data in the pooled reservoir sample to determine the optimal new partitioning criteria. It returns a new empty \syn with no node statistics.
	\item In parallel with (Step 1), the old synopsis is maintained under all insertions and deletions that happen during the optimization algorithm. Queries can still be answered with the old synopsis.
	\end{itemize}
    \item  (Blocking) Approximate node statistics are populated into the new synopsis using the pooled reservoir sample $S$ (note, that this will reflect any data that arrived during the optimization phase). This is the only blocking step in the re-initialization routine and new data and queries will have to wait until completion.
    \item The old synopsis is discarded.
	\item The system resamples a uniform sample of data from archival storage to be the new pooled reservoir sample. Queries and results can still be processed on the new synopsis even without a sample.
	\item Random samples of historical data are used to improve the node statistics in the background until a user-specified ``catch-up'' time. 
\end{enumerate}

This process is the key difference between an \prior and an \syn, where after catch-up the node statistics may be inexact.
However, this old data is propagated in a random order, which means that the SUM,COUNT,AVG values in each node will be unbiased estimates of their full data statistics.  The duration of the catch-up phase can be chosen by the user. For example, in our experiments, the catch-up phase does not stop until we get $0.1\cdot|\fullData|$ samples.
It is worth noting that queries close to the beginning of the catch-up phase will have a higher error, however queries towards the middle or the end of the catch-up phase will have a smaller error.
In Section~\ref{sec:re-partition}, we describe how to trigger re-initialization.
Furthermore, there is only one step (2) where the synopsis is unavailable to process queries and data (has the duration of 100s of milliseconds in our experiments).

%This multi-threaded re-initialization is also valuable in a warm-start setting. Imagine a scenario where \sys is deployed onto existing infrastructure with historical data and continuously arriving new data. In this case, even the initial construction of the first \syn synopsis will require a catch-up process.

\subsection{Answering Queries With a \syn}
\label{sec:estimators}
The query procedure does not access the entire data so the communication throughput (or the I/O operations) is zero.
The basic structure of the result estimator is the same as before, especially for the $R_{partial}$ partitions. However, there are a few key changes due to the nature of the catch-up phase. In \prior, for each partition in $R_{cover}$, we can compute an exact ``partial aggregate'' for the tuples in those partitions and combine the partial aggregates. In a \syn, this process changes
considering the estimations we get from the catch-up samples.
Overall, the estimation of a partition $R_i\in R_{cover}$ consists of i) estimation using the catch-up samples $H$ and the formulas of Section~\ref{sec:partTreeAQP}, ii) the exact statistics of the new inserted tuples in $R_i$, and iii) the exact statistics of the deleted tuples in $R_i$ (recall that the quantities in ii), iii) are stored and maintained as described in the Incrementally Maintaining Statistics in Section~\ref{sec:IncrMaintNodes}).
By taking the sum of i), ii) and subtracting iii) we get the unbiased estimation in partition $R_i$.


%\sk{I don't completely get this discussion...}
%In particular, we use the same estimates as in Section~\ref{sec:partTreeAQP} over the catch-up samples to get the statistics of the partitions in $R_{cover}$. 
%In the end, the final estimation of an aggregation function over a partition $R_i$ is given as the estimation using the node statistics plus the exact aggregation value of the new inserted items in partition $R_i$ minus the aggregation value of the deleted items in partition $R_i$ (recall the incrementally maintaining statistics in Section~\ref{sec:IncrMaintNodes}).
%Overall the estimation of a partition $R_i\in R_{cover}$ consists of a probabilistic estimation using samples $H$ and two exact deterministic values capturing the aggregation functions of the new inserted and deleted items in \syn. 
%This gives an unbiased estimation of COUNT, SUM, AVG in a partition $R_i$.

Let $H$ be the set of catch-up samples, $H_i\subseteq H$ be the subset of $H$ in partition $R_i$, and $h_i=|H_i|$. All basic notations are defined in Table~\ref{Table:Notation}.
The formulas for estimating COUNT and SUM queries in both $R_{cover}$, $R_{partial}$ from Section~\ref{sec:partTreeAQP} contain the factor $\frac{N_i}{m_i}$ or $\frac{N_i}{h_i}$, while the formulas for estimating the AVG contain the factor $\frac{N_i}{N_q}$. In \syn we do not have the exact values for $N_i$. Instead, we use an estimate of the size of the partition $R_i$ denoted by $\hat{N_i}$. In particular we use the catch-up samples $H$ to estimate $\hat{N_i}=\frac{h_i}{h}N$.
%to an approximate combination for AVG queries: $agg =  \sum_{P_i \in R_{cover}} P_i(q) \cdot  \textcolor{red}{\frac{\hat{N_i}}{\hat{N_q}}}$, where $\hat{N_i}$ is an estimate of the size of the partition $P_i$ and $\hat{N_q}$ is the total size in all relevant partitions of query $q$. This is because $N_i$ and $N_q$ are normally retrieved from the node statistics in the tree. Similarly, the weighting on the sample estimates for AVG queries change as well: $samp = \sum_{P_i \in R_{partial}} f(S_i) \cdot \textcolor{red}{\frac{\hat{N_i}}{\hat{N_q}}}$.

\subsubsection{Confidence Intervals}
While the estimators do not significantly change from an \prior to a \syn, the confidence intervals are calculated very differently. This is because there are now two sources of errors: estimation errors due to the stratified samples and estimation errors in the node statistics. Both these sources of errors have to be integrated into a single measure of uncertainty.
%To be able to analytically calculate these errors, we make a simplifying assumption to avoid having to deal with products of random variables.
%\emph{Large partition assumption. } We assume that the partition sizes are enough ($\Omega(\frac{m}{\alpha})$, where $\alpha$ is the reservoir-sampling rate) such that $\frac{N_i}{N_q}, \frac{N_i}{m_i}$ can be treated as deterministic values $\frac{\hat{N_i}}{\hat{N_q}}, \frac{\hat{N_i}}{m_i}$, as we had in the unbiased estimation above. This is an assumption similar to those made in previous AQP work~\cite{hellerstein1997online}.
%Once we make this assumption
Assuming that all partitions are large enough, the central limit theorem can be used to asymptotically bound the estimation error for SUM/COUNT/AVG queries. Informally, the central limit theorem states that this asymptomatic error is proportional to the square-root of the ratio of estimate variance and the amount of samples used $\propto \sqrt{\frac{var(est_i)}{m_i}}$.
We simply have to match terms to this formula for all sample estimates and all node estimates because both are derived from samples.

\mparagraph{Error in Node Estimates} First, let's account for all the uncertainty due to catch-up. Recall that $H$ is the set of catch-up samples we have considered so far and $H_i\subseteq H$ is the samples in partition $R_i$ with $h_i=|H_i|$. We note that we do not store the set $H$ or the subsets $H_i$, instead we only use the new catch-up samples to continuously improve the statistics we store in the nodes. Using the notation in the previous section, we can calculate the catch-up variance $\nu_c$:
\[
\nu_c(q) = \sum_{R_i\in R_{cover}} w_i^2\frac{var(\phi_q(H_i))}{h_i}
\]
where $w_i= \frac{\hat{N_i}}{\hat{N_q}}$ for AVG queries and $w_i=1$ for SUM/COUNT queries. Calculating $\phi_q(H_i)$ is straight-forward. We simply store additional information that allows us to efficiently calculate the variance. For any node $i$ of $\PASStree$ we store $h_i$, $\sum_{t\in H_i}t.a^2$, $\sum_{t\in H_i}t.a$.

\mparagraph{Error in Sample Estimates}
For a partition $R_i \in R_{partial}$, let $\samples_i\subseteq \fullData$ be the set of samples in $\samples$ that lie in partition $R_i$ and let $m_i=|\samples_i|$.
Like the catch-up variance, we can calculate the sample estimate variance $\nu_s$:
$$\nu_s(q) =  \sum_{R_i\in R_{partial}}w_i^2\frac{var(\phi_q(\samples_i))}{m_i}$$
We can calculate an overall confidence interval as:
$$\pm z \cdot \sqrt{\nu_c(q)  + \nu_s(q) } $$
where $z$ is a normal scaling factor corresponding to the desired confidence level, e.g., $z=1.96$ for 95\%. As before, $w_i= \frac{\hat{N_i}}{\hat{N_q}}$ for AVG queries and $w_i=1$ for SUM/COUNT queries.
In Appendix~\ref{appndx:varest}, we show analytically all formulas for computing the variance under different types of queries.

\iffalse
{\color{red}
\mparagraph{Communication throughput and I/O operations}
The query procedure of our system only accesses the partition tree stored in a local machine. Hence the communication throughput (or the I/O operations to access the full data) in the query procedure is zero.
}
\fi


==> DynamicPASS_ICDE FULLARXIV/dpt_old.tex <==
However, if we do not allow a full pass over $\fullData$ at the first construction of $\PASStree$, or after the first re-partition, we do not have the exact statistics in every node of the new tree $\PASStree$. After the construction of the main structure of $\PASStree$ we start a \emph{catch-up phase} where Dynamic PASS gets samples (in the background) from $\fullData$ to improve the statistics in the nodes of $\PASStree$. Given a sample $s$ from the catch-up phase we visit $\PASStree$ from the root to the corresponding leaf node updating the estimations of the statistics (as shown in Section~\ref{sec:estimators}) in $O(\ell)$ time. Let $H$ be the samples we get in the catch-up phase. We note that we do not store any samples from $H$ in Dynamic PASS, instead we only use them to improve the estimators of the nodes in $\PASStree$.  Since the catch-up phase runs in the background (in a different thread) there is no need to have a small duration. It is important to mention that Dynamic PASS can still answer aggregation queries and handle updates as the catch-up phase is running.


Since we do not have the exact statistics of the nodes as in the static PASS, we expect that the error of Dynamic PASS will be worse.
However, the catch-up phase is running  repeatedly (until it finishes) in the background so $|H|>>|\samples|$. Hence, we expect that queries that partially intersect leaf nodes will still have the higher error (longer confidence intervals). By optimizing a partition over the query with the largest error (Section~\ref{sec:partAlg}) we expect that the worst error of Dynamic PASS will only be slightly worse than the worst error of Static PASS leading to very accurate estimators.





As we mentioned in the issue (3), it might be possible that the current partition $\PASStree$ is not good enough for the updated set of samples $\samples$. For example, there might not be many samples in a leaf node (bucket) so the estimations are not robust, or the maximum confidence interval (error) is too large in $\PASStree$. In Section~\ref{sec:re-partition}
we describe an algorithm to decide when Dynamic PASS needs to re-partition. If a re-partition is needed we need to construct the new $\PASStree$ very fast so that the system is ready to support new queries as soon as possible. The algorithms in~\cite{liang2021combining} to construct a new partition  tree run in roughly $O(km)$ time. Ideally in the dynamic setting we do not want to spend $\Omega(m)$ time to construct the tree. In Section~\ref{sec:partAlg} (using the results of Section~\ref{sec:updateVar}) we propose new novel dynamic data structures with $O(m)$ space that allow us to construct the new partition tree $\PASStree$ in time roughly $O(k)$, which is optimal if a new partition with $k$ buckets needs to be constructed.


\subsection{Catch-Up Optimization}
In order to make PASS dynamic we need to propose non-trivial solutions to multiple problems.
Some of the core problems we need to consider are the following: (1) How to maintain a set of random samples $\samples$ over insertions and deletions? (2) How can we return estimators with provable confidence intervals under updates? (3) What if the current partition tree $\PASStree$ is not good enough (high error) with respect to the current set of samples $\samples$? Do we need to re-construct $\PASStree$? (4) How can we construct a new partition tree efficiently (in time that doe not depend on $m$)? (5) How can we maintain the statistics in the nodes?

In Section~\ref{sec:estimators} we show how to extend the estimators and the confidence intervals of static PASS for the Dynamic PASS. In a high level, we use estimators over the old data in $\fullData$ and we use exact statistics over the new inserted or deleted items.
Before the first re-partition if we allow to make a full pass over $\fullData$ as we construct $\PASStree$, someone can update all the exact statistics of the nodes in $\PASStree$ over insertions and deletions. Indeed, given a new insertion $t$ we can update the exact estimators from the root to the leaf node $u$ such that $t.p\in R_u$. Similarly we can update the aggregation functions in the nodes when a deletion happens in $O(\ell)$ time. 

==> DynamicPASS_ICDE FULLARXIV/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
We run our experiments on a Linux machine  with an Intel Core i7-8700 3.2GHz CPU and 16GB RAM. 

\subsection{Setup}
We generate query workloads of 2000 queries by uniformly sampling from rectangular range queries over the predicates. 
We then initialize a \sys instance with a user-specified sample rate, a catch-up ratio and a number of leaf nodes of the partition tree to compare with other baselines (these parameters directly control the Throughput, Query Latency, and Storage Size).

\subsubsection{Datasets}\sloppy
\textsf{Intel Wireless dataset}. The Intel Wireless dataset \cite{intelwireless_} contains 3 million rows of sensor data collected in the Berkeley Research lab in 2004. Each row contains measurements like humidity, temperature, light, voltage as well as the date and time each record was collected. 

\noindent \textsf{New York Taxi Records dataset}. The New York City Taxi Trip Records dataset \cite{nyctaxi} contains 7.7 million rows of yellow and green taxi trip records collected in January 2019. Each record contains information about the trip including
pickUpDateTime, dropOffDateTime, tripDistance, dropOffLocation, passengerCount, etc.
%\texttt{pickUpDateTime, dropOffDateTime, tripDistance, dropOffLocation, passengerCount}, etc.


\noindent \textsf{NASDAQ ETF Prices dataset}. The NASDAQ Exchange Traded Fund (ETF) Prices dataset\cite{nasdaq} contains 2166 ETFs traded in the NASDAQ exchange from April 1986 to April 2020. There are 4 million entries in the dataset and each entry contains the date, the volume of transactions of an ETF on the date, and 4 prices: the price of an ETF when the market opens and closes; the highest and the lowest of its daily price range.

\subsubsection{Metrics and ground truth}
We report the wall-clock latency and the throughput, i.e. number of requests (query/data) processed per second. 
To measure the accuracy of the system,  we report the 95 percentile of the relative error which is the difference between ground truth and estimated query result divided by the ground truth. 
We define the ground truth to be w.r.t all the tuples available when the query arrives, i.e. the true results reflect all insertions and deletions up to its arrival point.
To make sure our experiments are deterministic, we fix this sequence up-front and ensure they are the same for each baseline.

\subsubsection{Baselines} 
All of these baselines are tuned to roughly control for query latency.

\vspace{0.5em}

\noindent \textbf{Reservoir Sampling (RS) and Stratified Reservoir Sampling (SRS).} We construct a uniform sample of the entire data set which is maintained using the reservoir sampling algorithm~\cite{vitter1985random}. We use a variant of RS first designed for the AQUA system that handles both insertions and deletions~\cite{gibbons2002fast}\footnote{Due to its age, a direct comparison with AQUA was not feasible}. Unless otherwise noted, we use a 1\% sample of data. For stratified seservoir sampling, the strata is constructed using a equal-depth partitioning algorithm. 


\noindent \textbf{DeepDB. }  We also compare with a machine learning-based baseline called \textsf{DeepDB}\cite{hilprecht2019deepdb}. DeepDB achieves state-of-the-art AQP results in the static setting, and we chose it as a baseline since it has limited support for dynamic data. In our baseline, DeepDB trains on 10\% of the data. We set this to be equivalent to the ``catch-up'' sampling in \syn.

\noindent \textbf{Dynamic Partition Tree-Only (\syn). } We compare with a baseline of only using a single \syn synopsis without online optimization. This synopsis is constructed once and then used for the duration of the experiment. Unless otherwise noted there are 128 leaf nodes in a balanced binary tree, the leaf nodes are associated with 1\% samples of their respective strata, and the catch-up sampling rate 10\% of the data.

\noindent \textbf{\sys. } Finally, we evaluate the full-featured \sys system. This includes a \syn and also performs re-partitioning if needed. Unless otherwise noted there are 128 leaf nodes in a balanced binary tree, the leaf nodes are associated with 1\% samples of their respective strata, and the catch-up sampling rate 10\% of the data.

\vspace{0.5em}

The storage costs of the baselines on the NYC Taxi dataset given the typical setting (128 leaf-nodes, 10\% catch-up rate, and 1\% sample rate) are: reservoir sampling baseline takes about 5MB, \sys and \syn takes about 6MB, a DeepDB baseline trained with 10\% of the data is about 60MB.
%sys is over-estimated using 1k for each node to store the summaries.
\iffalse
We use a simple diagram to better demonstrate how an experiment is conducted: i.e., how the systems are initialized and when are the queries evaluated, etc. For example, in the example workflow shown in Figure \ref{wf:example}, a baseline is initialized with the first 10\% of the dataset, then repeatedly another 10\% of data is inserted followed by a 1\% deletion. The same set of queries are evaluated every time the insertions and deletions are finished and the workflow stops when the entire dataset is inserted.
\begin{figure}[ht]
\centering
\digraph[scale=0.4]{abcdef}{
      rankdir=LR;
      a -> b -> c -> d -> e
      d -> b
      a [label="start(10\%)"]
      b [label="+10\%"]
      c [label="-1\%"]
      d [label="query"]
      e [label="end"];
   }
\caption{An example workflow.}
\label{wf:example}
\end{figure}
\fi

\subsection{Accuracy}
\label{sec:end-to-end}

% 1% sample rate for RS and SRS, JanusAQP: 10\% catchup + 1% sample rate, DeepDB: 10\% sample for training

\begin{table*}[ht]
    \caption{Median relative error (\%) of 2000 SUM random queries and average query latency (ms/query) over three datasets.}
    \label{tbl:macro-acc-latency-vs-deep-rs}
   % \scriptsize
    \centering
    
    \begin{tabular}{|c|}
        \hline
        \multicolumn{1}{|c|}{---}\\
        \hline
        Approach \\\hline
        % OnlinePASS   \\
        \sys   \\ %1x
        DeepDB   \\ %2x
        RS    \\
        SRS    \\\hline
    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{Intel (\%)}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.67  & 0.62 & 0.33 \\        
        1.5 & 1.7 & 0.8\\
        2.1 & 1.6 & 1.3  \\
        1.3 & 1.3 & 1.2  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{NYC (\%)}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.48  & 0.22 & 0.2 \\        
        4.7 & 4.7 & 4.7\\
        3.4 & 2.1 & 0.94  \\
        2.4 & 1.2 & 0.95  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{ETF (\%)}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        5  & 4.3 & 2.3 \\   
        -  & - & - \\   
        16  & 9.8 & 8.6 \\   
        10  & 8.2 & 8 \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{Intel (ms/query)}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.19  & 0.31 & 0.63 \\        
        0.6 & 0.6 & 0.6\\
        2.5 & 6.3 & 13.2\\
        3.1 & 6 & 10.7  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{NYC (ms/query)}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.27  & 0.57 & 0.97 \\        
        0.6 & 0.6 & 0.6\\ 
        4.7 & 14.2 & 30.6\\
        4.6 & 14.7 & 25.3  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{ETF (ms/query)}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.14  & 0.28 & 0.46 \\        
        0.6  & 0.6 & 0.6 \\   
        2.58  & 6.8 & 13 \\   
        2.66 & 5.2 & 12.7  \\\hline

    \end{tabular}
    
    % Xi: same set of queries evaluated at different time.

\end{table*}


We first evaluate the end-to-end performance of \sys and the baselines on a 1d problem (1 predicate attribute).
For the NYC Taxi dataset, we use the \texttt{pickUpTime} attribute as the predicate attribute and the \texttt{tripDistance} attribute as the aggregate attribute; for the ETF dataset, we use the \texttt{volume} attribute as the predicate attribute and the \texttt{close} attribute as the aggregate attribute; for the Intel Wireless dataset, we use the \texttt{time} and \texttt{light} attributes as predicate and aggregate attribute respectively.

We start with 10\% of the data in Kafka which is used by the baselines for initialization (simulating historical data). We incrementally add 10\% more data in increments (simulating new data arrival).
After every 10\% increment, we re-train the model for DeepDB and re-initialize the DPT used by \sys. 
We report results when 20\%, 50\%, and 90\% of the rows from each dataset are inserted into the system. The median relative error and the corresponding average query latency can be found in Table \ref{tbl:macro-acc-latency-vs-deep-rs}.

We can see that \sys has the overall best accuracy while controlling for query latency.
We note that the accuracy of DeepDB is stable as a function of progress. This is because as a learned model DeepDB has a roughly fixed resolution of the data (it does not increase the number of parameters as more data is inserted).\footnote{We omit the results of DeepDB on the ETF dataset in Table \ref{tbl:macro-acc-latency-vs-deep-rs} due to very large error ($>$ 1000\%) for SUM queries while the error of COUNT queries is reasonable.} These findings are consistent with results from \cite{liang2021combining}. The accuracy of RS and SRS improves at a cost of a higher query latency. %(1\% sample of the entire dataset). 

\iffalse
\begin{table*}[ht]
    %\small
    \centering
    
    \begin{tabular}{|c|}
        \hline
        \multicolumn{1}{|c|}{---}\\
        \hline
        Approach \\\hline
        % OnlinePASS   \\
        \sys   \\ %1x
        DeepDB   \\ %2x
        RS    \\
        SRS    \\\hline
    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{Intel}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.67\%  & 0.62\% & 0.33\% \\        
        1.5\% & 1.7\% & 0.8\%\\
        2.1\% & 1.6\% & 1.3\%  \\
        1.3\% & 1.3\% & 1.2\%  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{NYC}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.48\%  & 0.22\% & 0.2\% \\        
        4.7\% & 4.7\% & 4.7\%\\
        3.4\% & 2.1\% & 0.94\%  \\
        2.4\% & 1.2\% & 0.95\%  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{ETF}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        5\%  & 4.3\% & 2.3\% \\   
        -  & - & - \\   
        16\%  & 9.8\% & 8.6\% \\   
        10\%  & 8.2\% & 8\% \\\hline

    \end{tabular}
    
    % Xi: same set of queries evaluated at different time.
    \caption{Median relative error of 2000 SUM random queries over three datasets.}
    \label{tbl:macro-acc-vs-deep-rs}
\end{table*}

\begin{table*}[ht]
    %\small
    \centering
    
    \begin{tabular}{|c|}
        \hline
        \multicolumn{1}{|c|}{---}\\
        \hline
        Approach \\\hline
        \sys   \\ %1x
        DeepDB   \\ %2x
        RS   \\ %2x
        SRS    \\\hline
    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{Intel}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.19  & 0.31 & 0.63 \\        
        0.6 & 0.6 & 0.6\\
        2.5 & 6.3 & 13.2\\
        3.1 & 6 & 10.7  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{NYC}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.27  & 0.57 & 0.97 \\        
        0.6 & 0.6 & 0.6\\ 
        4.7 & 14.2 & 30.6\\
        4.6 & 14.7 & 25.3  \\\hline

    \end{tabular}
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{ETF}\\
        \hline
        0.2 & 0.5 & 0.9\\\hline
        0.14  & 0.28 & 0.46 \\        
        0.6  & 0.6 & 0.6 \\   
        2.58  & 6.8 & 13 \\   
        2.66 & 5.2 & 12.7  \\\hline

    \end{tabular}
    
    \caption{Average query atency (ms/query) over three datasets.}
    \label{tbl:macro-latency-vs-deep-rs}
\end{table*}




\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{exp-figures/end2end-taxi-2k-p95re-cost-128-nodpt.pdf}
  \caption{We compare the accuracy (left plot) and re-optimization cost (right plot) of \sys with DeepDB and reservoir sampling on the NYC Taxi dataset. }
  \label{fig:end2end}
\end{figure}

\fi

\subsection{Online Performance}
 We populate Kafka with the first $p$ percent of the NYC Taxi dataset ($p$ varies from 10 to 90). Like before, we initialize \sys on the first 10\% of data and then incrementally add increments of 10\% more. In this experiment, we construct a mixed update workload of both insertions and deletions.
On the left plot of Figure \ref{fig:thruputopt}, we show the throughput of handling insertions and deletions using a pool of 12 threads. We can see the performance of \sys is quite stable and does not change with the size of existing data or the amount of data that have been processed. For each insertion and deletion, we simply find the target node in $O(\log(k))$ and modify the summary. Even though a larger reservoir size increases the overhead of manipulating the samples for reservoir sampling, the increased overhead is unnoticeable. This is because the stratum stored in each node is $\frac{1}{k}$ of the reservoir, and each stratum is independent with others and race condition only happens if two workers are working on the same node. 

On the right plot of Figure \ref{fig:thruputopt}, we show the re-optimization time cost in seconds by \sys and DeepDB. The cost to initialize \sys increases with the number of tuples stored in Kafka but it is still much cheaper than DeepDB. It is worth noting that the re-optimization cost of DeepDB is the cost of re-training instead of incremental training. This is mostly due to the constraint of the API exposed by DeepDB, and we observe that re-train a model with 2$n$ samples is faster than train a model with $n$ samples then incrementally train another $n$ samples.
The results suggest that complex, learned synopses are not ideal in the dynamic setting.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{exp-figures/thruput-reopt.pdf}
  \caption{We evaluate the throughput of \sys when handling insertions and deletions in multi-threaded mode. We also compare the re-optimization cost with DeepDB.}
  \label{fig:thruputopt}
\end{figure}

\iffalse
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{exp-figures/end2end-taxi-2k-throughput-128.pdf}
  \caption{We evaluate the throughput (left plot) of \sys when handling insertions and deletions in multi-thread mode. We also compare the re-optimization cost (right plot) with DeepDB.}
  \label{fig:throughput}
\end{figure}
\fi

\subsection{Handling Deletion}
We construct a \sys instance with the 50\% percent of each dataset, then we delete the last $p$\% of data of the first 50\% ($p$ varies from 1\% to 9\%). After \sys process all the deletions, a query workload of 2000 random queries is evaluated and we record the median relative error of the 2000 queries. We use the data that remains in the system to compute the ground truth, e.g., for $p=1\%$, the ground truth is computed with the first 49\% of each dataset. 

Results can be found in Figure \ref{fig:del3in1}, we notice that the relative error is relatively stable when we vary the deletion percentage. This is because the tuples that are being deleted are uniformly distributed over the predicate attributes of the query workloads, i.e. the deletion would occur in each leaf node of the DPT with roughly the same probability, therefore, the DPT without re-optimization works reasonably well.
In another experiment we artificially generate deletions that are skewed to demonstrate scenario where re-optimization is needed, details can be found in Sec. \ref{sec:exp-del}.


\begin{figure}[t]
  \centering
  \includegraphics[scale=0.22]{exp-figures/del0.4-0.5.pdf}
  \caption{Median relative error of \sys varying the amount of deletions from 1\% to 9\% over three datasets.}
  \label{fig:del3in1}
\end{figure}
\iffalse
\begin{table*}[ht]
    \centering
    \begin{tabular}{|c|}
        \hline
        Dataset \\\hline\
        IntelWireless   \\ 
        ETF    \\
        NYCTaxi    \\\hline
    \end{tabular}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        1\% & 2\% & 3\% & 4\% & 5\% & 6\% & 7\% & 8\% & 9\% \\\hline
        0.36\% &
        0.50\% &
        0.39\% &
        0.42\% &
        0.61\% &
        0.36\% &
        0.42\% &
        0.50\% &
        0.45\% 
        \\ 
        4.57\% &
        3.57\% &
        2.96\% &
        3.89\% &
        3.26\% &
        3.91\% &
        3.12\% &
        3.58\% &
        4.01\% 
        \\ 
        0.35\% &
        0.37\% &
        0.41\% &
        0.34\% &
        0.25\% &
        0.25\% &
        0.29\% &
        0.26\% &
        0.26\% 
        \\\hline

    \end{tabular}
    
    % Xi: same set of queries evaluated at different time.
    \caption{\onethree{Median relative error of \sys after process different amount of deletions.}}
    \label{tab:macro-acc-vs-deep-rs}
\end{table*}
\fi

\subsection{The Catch-up Phase}
In this experiment, we study how the catch-up phase can impact the accuracy and performance of the entire system.

\subsubsection{Accuracy}
We use the entire Intel wireless dataset as the existing data. We compare a set of \sys(128, $c$, 1\%) instances where the catch-up goal $c$ varies from 1\% to 10\% with a step of 1\%. When each \sys instance reaches the catch-up goal, we use it to evaluate the same set of 2000 random queries generated using the light attribute as the aggregate attribute and the time attribute as the predicate attribute.

The results can be found in the left plot of Figure \ref{fig:intel-catchup-ratio-vs-nx}. As a reference, we also show the accuracy of an RS baseline with 1\% sample rate. We notice that \sys(128,1\%,1\%) has no advantage against the RS baseline because neither the samples nor the summaries built during catch-up could provide better accuracy. As we increase the catch-up ratio, we can see an improvement in accuracy because the quality of the summaries built by the catch-up phase improved. Comparing with the expensive offline pre-processing used in \cite{liang2021combining}, we believe the catch-up phase is a better alternative that provides another knob to tune the tradeoff between accuracy and cost.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{exp-figures/catchup-intelfull-2k-p95re-time-128.pdf}
  %\includegraphics[width=0.8\linewidth]{exp-figures/ICDE/catchup-intelfull-2k-p50re-time-128.pdf}
 % \includegraphics[width=0.8\linewidth]{exp-figures/ICDE/catchup-intelfull-2k-mean-re-time-128.pdf}
  \caption{Varying the catch-up goal from 1\% to 10\% of the data, we evaluate the accuracy of \sys (left plot) and the time cost of the catch-up phase (right plot).}
  \label{fig:intel-catchup-ratio-vs-nx}\vspace{-1em}
\end{figure}

\subsubsection{Overhead}
The overhead of the catch-up phase comes from two sources: the loading and processing of the samples. 
We distinguish and measure the two types of overhead in terms of their time cost. Data loading time measures the time spent on calling the Kafka \code{poll()} API, transferring the data, and ETL operations that are necessary to prepare the data for \sys to process. It is worth noting that the data loading cost is part of the essential cost that occurs in all systems and is usually less relevant to the core design of the system but more relevant to the design of interfaces. For example, with a different interface, instead of dealing with the strings from Kafka that can be expensive to parse, the system could use Protocol Buffers\cite{protobuff} for more efficient data exchanging or even offload some of the ETL duties to the client-side as described in \cite{ding2021ciao}. On the other hand, the data processing time stands for the time taken by \sys to analyze the data then accordingly modify internal data structures that will be used for query processing.  

Results can be found in the right plot of Figure \ref{fig:intel-catchup-ratio-vs-nx}. We can see that the data processing with a single thread takes less than 1.5 seconds for a catch-up ratio of 10\%, which is equivalent to a throughput of processing 160,000 tuples per second. Furthermore, the data loading cost is much higher than the data processing cost and we believe the data loading cost can be further improved by more engineering efforts and techniques such as client-assisted data loading\cite{ding2021ciao}.


\reviewtwo{
\subsection{Dynamic Query Templates}
\label{subsection:robustness}
}

\reviewtwo{
In this section, using the NYC Taxi dataset, we conduct experiments to demonstrate the robustness of \sys. In particular, we implement the heuristic way of \sys to handle new query templates, as described in Subsection~\ref{subsection:discussion}. We explore the error considering all three cases: Different predicate attributes, different aggregation attribute, and different aggregation function.
}

\reviewtwo{
First, we consider the case where \sys is constructed using one predicate attribute but the query uses another attribute as predicate attribute. In Subsection~\ref{subsection:discussion} we proposed three ways to handle it. Here we implement the simpler way where we apply uniform sampling using the samples $\samples$ which leads to higher query latency similar to what we observed for RS in Table \ref{tbl:macro-acc-latency-vs-deep-rs}.  The results can be found in the left plot of Figure \ref{fig:p95-3in1}: the PickupOverPickup baseline is the case where the query and \sys both use the PickupTime attribute as predicate attribute; the DropoffOverDropoff baseline is the case where the query and \sys both use the DropoffTime attribute as predicate attribute; lastly, the DropoffOverPickup baseline is the case where the query use the DropoffTime attribute as predicate attribute while \sys is constructed using PickupTime as predicate attribute. We observe that when  the two attributes differs (DropoffOVerPickup) we have the highest error (but still it happens to be quite competitive). After a re-partitioning with respect to the new predicate attribute the high accuracy can be restored (DropoffOverDropoff). Even though we drew three curves over the entire progress, we assume that the system first considers PickupOverPickup between $[0.1-0.3)$ (cycles), then DropoffOverPickup between $[0.3-0.6)$ (stars), and finally DropoffOverDropoff between $[0.7-0.9]$ (triangles). We present all values over the three curves to show all the details. This is also the case in all plots of Figure~\ref{subsection:discussion}.
}

% XI: would the reader argue that the case of use sample only is pretty good already? Some elaboration on sample only baseline here to justify?

\reviewtwo{
Second, we consider the case where \sys is constructed using one aggregation attribute but the query uses a different aggregation attribute. In Section~\ref{sec:partAlg}, we described how the aggregation attribute is used by our partitioning algorithm while constructing \sys. In this experiment, we show how the change of aggregation attribute affects the performance of \sys. The result can be found in the middle plot of Figure \ref{fig:p95-3in1} where we show two baselines indicating whether the aggregation attribute used by \sys is the same with the aggregate attribute of the query. We can see the accuracy of the two baselines are quite close, which suggests that \sys is quite robust over the change of the aggregation attribute.
}

% XI: for Same: both use trip_distance, for Diff: sys use PickupLocationID, query use trip_distance

\reviewtwo{
Finally, we study how \sys performs over different aggregation functions. As we described earlier, SUM, CNT and AVG are all part of the statistics we keep and maintain in the partition tree therefore no additional effort is required to take care of a change in aggregation function. Results in the right plot of \ref{fig:p95-3in1} suggest all the three aggregate functions can achieve good accuracy, which also implies other aggregate functions such as STDDEV that can be composed using SUM and CNT would also perform well.
}

\reviewtwo{Overall, we show that our system can support different query templates with low error even with the heuristic way that stores and maintains only one partition tree.}


\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{exp-figures/ICDE/3in1-p95.pdf}
  \caption{\reviewtwo{We evaluate the robustness of \sys over three scenarios where the predicate attribute, the aggregate attribute, and the aggregate function used by the query workload might change from the ones that are used to construct \sys.}}
  \label{fig:p95-3in1}\vspace{-1em}
\end{figure}

\subsection{Multi-dimensional Query Templates}
Next, we investigate the performance of \sys with multi-dimensional queries on the NASDAQ ETF Prices dataset. We randomly generate 2000 queries from a 5-D query template that uses the volume attribute as the target attribute, the date attribute and the 4 price attributes as predicate attributes. We perform the same workflow as we did in Section \ref{sec:end-to-end}. We first compare the median relative error of \sys(256,10\%,1\%) with DeepDB and the results can be found in the left plot of Figure \ref{fig:etf-kdtree}. We notice that the accuracy of \sys is better than DeepDB but the relative error increases for both. This is because multi-dimensional queries are usually more selective. Also, because the queries are generated using the entire dataset, we notice that many of the ground truths generated using the first 20\% of the data are 0s. Therefore, in the experiment, we start with 30\% of the data. 
On the right plot of Figure \ref{fig:etf-kdtree}, we can find the re-optimization cost of \sys is lower than DeepDB but is more expensive than in the 1D setting. While the increase of dimensions can indeed make it more expensive to process the samples we fetched during catch-up, we believe the re-optimization cost can be further improved with more engineering efforts. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{exp-figures/end2end-etf-2k-p50re-cost-256.pdf}
  \caption{We compare the median relative error and the re-optimization cost of \sys with DeepDB on multi-dimensional queries. 
  %Both perform re-optimization after every 10\% insertion then evaluate the same set of queries.
  %XI: p95 and mean not available (don't have access to deepdb data anymore after graduate because it was on another machine.)
  }
  \label{fig:etf-kdtree}
\end{figure}


\subsection{Re-partitioning}
\label{sec:exp-del}
In the first experiment, using the NYC Taxi dataset, \sys performs a periodic re-partitioning after every 10\% insertions. For comparison, the \syn baseline does not perform any re-partitioning and we evaluate the accuracy. 
We deliberately skew the insertions by sorting on \texttt{pickUpDateTime} so that new insertions would hit a small number of partitions.
The results are illustrated in Figure \ref{fig:repartition}(left), we can see the relative error of \syn increases drastically due to a partition tree that becomes more and more imbalanced with new insertions. With periodic re-partition, \sys keeps the accuracy at a controlled level.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{exp-figures/ICDE/end2end-taxi-2k-p95re-repartition.pdf}
  %\includegraphics[width=0.8\linewidth]{exp-figures/ICDE/end2end-taxi-2k-p50re-repartition.pdf}
 % \includegraphics[width=0.8\linewidth]{exp-figures/ICDE/end2end-taxi-2k-mean-re-repartition.pdf}
  \caption{We compare the accuracy of \sys and \syn in two scenarios that cause imbalanced partition trees.}
  \label{fig:repartition}
\end{figure}

In the second experiment, we use the \texttt{pickupTimeOfDay} as the predicate attribute. Because the dataset is randomly distributed
over the \texttt{pickupTimeOfDay} attribute, the insertions are not skewed as in the previous setting. 
To demonstrate a situation where a re-partition is triggered by deletions, we randomly choose 10\% of the nodes and we randomly delete half of the samples that belong to these nodes then we insert the next 10\% data. After the insertion, the re-partition will be triggered for \sys. For comparison, we use a \syn baseline that does not perform any re-partition. We perform the same operations to the leaf nodes of the \syn baseline then we evaluate the same set of queries.
The results can be found in the right plot of Figure \ref{fig:repartition}, we can see the relative error of \syn increases due to the imbalanced partition tree while the error of \sys drops because of re-partition.

% Xi: note to self, usually, it is the case that the accuracy of sys increases with the size of reservoir for the same dataset which is the case for the 2nd repartition experiment and experiments before. however, it is not the case for repartition experiment 1, because the skewed insertion hurt the accuracy and countered the benefit of an increasing reservoir, therefore the controlled accuracy is a good result comparing with an otherwise increased error.

%the repartition/reinitialization also improves the reservoir size but it is still somewhat a fair comparision because DPT process every new insertions while \sys only process with catch-up rate


\subsection{A More Efficient Partitioning Algorithm}
% As mentioned earlier, we borrow the idea of combining aggregates with sampling from PASS\cite{liang2021combining} and propose a couple novel contributions that enable \sys to handle insertions and deletions. Because PASS is not designed to work with dynamic data, it is not end-to-end comparable to \sys and we study the main contributions that enable \sys to work with dynamic data in previous experiments.

In Section \ref{sec:partAlg}, we propose a binary search-based (BS-based) partitioning algorithm for 1 dimension that is much more efficient. In this experiment, we compare the accuracy and time cost of the BS-based algorithm with the dynamic programming-based partitioning algorithm used by PASS on the Intel Wireless dataset. We implement the BS-based algorithm in Python in our code base of PASS for a fair comparison. We measure the time cost in seconds of each partitioning algorithm given different number of partitions, we also compare the median relative error of the PASS variation over 2000 randomly generate queries.

\begin{table}[t]
\caption{We compare our new binary search-based (BS) partitioning algorithm with the dynamic programming-based (DP) algorithm proposed in~\cite{liang2021combining} on the Intel dataset.}
\label{tbl:partition}
\footnotesize
\centering
\begin{tabular}{|cl|l|l|l|l|}
\hline
\multicolumn{1}{|l}{} &      & 16    & 32    & 64     & 128    \\ \hline
\multirow{2}{*}{Partition Time (s)}       & DP & 16    & 22    & 382    & 6349   \\
                                          & BS  & 0.3   & 0.3   & 0.4    & 1.6    \\
\multirow{2}{*}{Median RE (CNT)}        & DP & 0.2\% & 0.1\% & 0.05\% & 0.04\% \\
                                          & BS  & 0.6\% & 0.4\% & 0.1\%  & 0.1\%  \\
\multirow{2}{*}{Median RE (SUM)}          & DP & 0.2\% & 0.1\% & 0.07\% & 0.05\% \\
                                          & BS  & 1\%   & 0.9\% & 0.2\%  & 0.2\%  \\
\multirow{2}{*}{Median RE (AVG)}          & DP & 0.2\% & 0.1\% & 0.08\% & 0.05\% \\
                                          & BS  & 1\%   & 0.7\% & 0.2\%  & 0.15\% \\ \hline
\end{tabular}
\end{table}
The result can be found in Table \ref{tbl:partition}. We vary the number of partitions from 16 to 128, as we increase the number of partitions, the sample size used by the algorithms also increase. We notice that the time cost of the DP-based algorithm increase drastically with the number of partitions while the time cost of the BS-based algorithm increase slightly.
On the accuracy side, the DP-based algorithm does lead to a lower error but the BS-based algorithm also introduce good accuracy. Overall, we believe the BS-based algorithm is more scalable than the DP-based algorithm and it provides favorable trade-off between cost and accuracy. 



% \subsubsection{Online} 
% PASS is not designed to handle dynamic data but a reasonable and straightforward improvement that can make it somewhat 'dynamic' is to use the new insertions and deletions to improve the statistics in the partition tree -- which behaves like a simplified \sys, i.e. without reservoir sampling and re-partitioning. We call this baseline DPASS and compare with \sys in this experiment.



==> DynamicPASS_ICDE FULLARXIV/implementation.tex <==
\section{System Architecture}
\label{sec:implementation}
In this section, we describe the \sys architecture.
\vspace{-0.5em}
\subsection{Construction and Optimization API}
\label{subsection:constructAPI}
\reviewtwo{
First, we overview how users construct synopsis data structures in \sys.
In order to simplify the description of our system, for now, we consider that
unlike systems like BlinkDB~\cite{agarwal2013blinkdb}, \sys does not use a single synopsis to answer all queries. Instead, \sys constructs a different synopsis for each different query template that the user is interested in. In Subsection~\ref{subsection:discussion} we describe how we can construct a single synopsis that can answer different query templates.
Much like index construction in a database, users choose which attributes to include in the synopsis structure. Each synopsis can answer query templates of the following form:}
\begin{verbatim}
SELECT SUM/COUNT/AVG/MIN/MAX(A) FROM D
WHERE Rectangle(D.c1,...,D.cd)
\end{verbatim}
\reviewtwo{
where $A$ is an aggregation attribute and $c_1,...,c_d$ are predicate attributes used in some rectangular predicate region (a conjunction of $>,<,=$ clauses). The \textbf{dimensionality} of a synopsis is the number of predicate attributes $d$.
To construct a synopsis, the user must define the following basic inputs:
\vspace{-0.5em}
\begin{itemize}
    \item \textbf{Aggregation Attribute and Aggregation Function. } An attribute $A$ that is the primary metric for aggregation. 
    \item \textbf{Predicate Attributes. } A collection of $d$ columns $c_1,...,c_d$ that are used to filter the data prior to aggregation. 
    \item \textbf{Memory Constraint. } The maximum amount of space that the synopsis can take.
\end{itemize}
The user can also optionally define a query processing constraint, i.e, the maximum bytes of data that the system should process in answering a query. %If the user does not define such a constrain, \sys can automatically decide an upper bound on query processing constraint as we also describe in Subsection~\ref{}.
Finally, the user has the option to set a historical data limit which is how much historical data to include in the synopsis, i.e., the earliest time-step of data included in the system.
In Subsection~\ref{subsection:discussion} we also show how \sys uses these constraints to generate a synopsis with low error.
}

Beyond these basic knobs that are relevant to most AQP systems, there are two other considerations discussed in this paper:  

\vspace{0.25em} \noindent \textbf{Catch-Up Processing. } Constructing a synopsis will require some amount of computational time. While incremental maintenance might be efficient, constructing the initial synopsis $S^{(0)}$ from the initial database state $\fullData^{(0)}$ might be very expensive if there is a significant amount of initial data. As the initial $S^{(0)}$ is being constructed new data will arrive, and the system will require additional processing to catch up. \sys optimizes the catch-up process using a multi-threaded system and approximate internal statistics for the partition tree. This process minimizes the amount of time where the system is unable to process new data or queries. The user decides how much processing to expend during catch up, the quicker the system is ready, the higher the error will be.

\vspace{0.25em} \noindent \textbf{Throughput. } The maximum data throughput is the maximum rate of insertions and deletions that the system can support. Throughput depends on the complexity of the synopsis used.

\subsection{Data and Query API}
For processing queries and data, we adopt the PSoup architecture where both queries and data are streams~\cite{chandrasekaran2003psoup}.
\sys supports three types of requests: insertion of a new tuple, deletion of an existing tuple and querying of the existing tuples. Thus, there are three Kafka topics \textsf{insert(tuple)}, \textsf{delete(tuple)}, and \textsf{execute(query)}.

The use of Kafka, with its timing and delivery guarantees, simplifies the query processing semantics.
The system will process the incoming stream of queries in order. Each query will have an arrival time $i$, which is the current database state at the time at which the query is issued. Therefore, we define $q^{(i)}_j$ as the $j$th query in the sequence that arrives at database state $i$. Query results should reflect all of the data that has arrived until the time point $i$.

\iffalse
\subsection{Summary and Algorithmic Contributions}
To summarize, the usage of \sys can be thought of as a life cycle. (1. Initialization) The user triggers synopsis construction through an API call. (2. Catch-Up) The system will online construct the synopsis while managing new data arriving into the system. 
(3. Query/Data Processing) Then, \sys is ready to process requests of insertions, deletions, and queries. (4. Re-Initialization) As \sys processes more updates, the data or query workload could drift requiring re-partitioning. This procedure re-enters the initialization phase.

Throughout the rest of the paper, we present technical contributions throughout this synopsis life cycle:
\vspace{-0.3em}
\begin{itemize}
    \item \textbf{Dynamic Partition Trees (Section \ref{sec:dpt})} The core data structure in \sys is called a dynamic partition tree (\syn). This data structure aggregates data at multiple levels of resolutions and associates some of the aggregates with stratified samples. The size of the tree (i.e., depth and width) can be changed to tradeoff accuracy at the cost of increased storage and throughput.
    The sampling rate at the leaf nodes can be adjusted to tradeoff query latency with accuracy.
    \item \textbf{Warm-Start Deployment (Section \ref{sec:catchup})} Next, we present a multi-threaded technique that allows \syn synopses to be deployed in dynamic environments accounting for new data that might arrive during their construction. This component crucially allows for either partial or full online re-partitioning and re-balancing of the data structure. 
    \item \textbf{Minimum Variance Partitioning (Section \ref{sec:partAlg})} We describe a new, efficient algorithm for selecting the \syn tree structure that minimizes the worst-case estimation error. 
\end{itemize}
\fi

==> DynamicPASS_ICDE FULLARXIV/introduction.tex <==
\section{Introduction}
Approximate query processing (AQP) studies principled ways to sacrifice query result accuracy for faster or more resource-efficient execution~\cite{chaudhuri2017approximate, garofalakis2001approximate}.
AQP systems generally employ reduced-size summaries, or ``synopses'', of large datasets that are faster to process.
The simplest of such synopsis structures are histograms and samples~\cite{cormode2011synopses, liang2021combining, agarwal2013blinkdb, lazaridis2001progressive}, but many others have been proposed in the literature.
More complex synopses are more accurate for specific types of queries~\cite{walenz2019learning}, specific data settings~\cite{poepselland}, or even are learned with machine learning models~\cite{yang2019deep, hilprecht2019deepdb, ma2021learned}. 
AQP is particularly interesting and challenging in a  \textbf{dynamic data setting}, where a dataset is continuously modified with insertions and deletions~\cite{garofalakis2001approximate, olma2019taster, acharya1999aqua}.
In this setting, hereafter denoted as DAQP, any synopsis data structures have to be continuously maintained online.

As an example use-case, consider a database aggregating per-stock order data for the NASDAQ exchange~\cite{nasdaqbv}.
Suppose, that we would like to build a low-latency SQL interface for approximate aggregate queries over the past seven days of order data. 
On a typical day, there are 25M new orders that correspond to trades that are placed by brokers (up to 70,000 orders in any given second).
A decent fraction of these orders are eventually canceled or prematurely terminated, for a variety of financial reasons.
Thus, this database is highly dynamic with a large volume of new insertions (new orders) and a small but significant number of deletions (canceled orders).
This paper explores such scenarios with similar motivating applications in internet-of-things monitoring and enterprise stream processing.

Simple synopses like 1D histograms and uniform samples are easy to maintain dynamically. However, such structures are often inaccurate in high-dimensional data and selective query workloads. More complex synopses structures, e.g, ~\cite{yang2019deep,liang2021combining} can be optimized for a particular instance (dataset and query workload),  but are generally harder to maintain online.
For example, recently proposed learned synopses require expensive retraining procedures which limit insertion/deletion throughput~\cite{yang2019deep, hilprecht2019deepdb, ma2021learned}.
Even classical stratified samples may have to be periodically re-optimized and re-balanced based on query and workload shifts~\cite{agarwal2013blinkdb}.
These, expensive (re-)initialization procedures can significantly hurt insertion throughput, and accordingly, almost all existing AQP systems focus on the static data warehousing setting\footnote{A notable exception being the AQUA project~\cite{acharya1999aqua} from 20 years ago.}.
Unfortunately, the existing techniques that \emph{are} designed for dynamic data, such as sketches and mergeable summaries~\cite{gan2020coopstore, agarwal2012mergeable,poepselland, cormode2011synopses, gan2020coopstore, agarwal2012mergeable}, often cannot handle arbitrary deletions or aggregation queries with arbitrary predicates easily.

\reviewone{
In particular, traditional sketch techniques~\cite{cormode2011sketch, cormode2011synopses} focus on frequency, distinct values, and quantile problems. They do not handle arbitrary range queries with low error guarantees and they only consider updates in the streaming setting, i.e. they do not handle arbitrary insertions and deletions.
Our system has a few similarities with high dimensional histograms which is another type of sketching that has been used for aggregation queries. We construct a space partitioning and we store some statistics to answer queries, which is also the case for high dimensional histograms. However, we propose a dynamic method that combines partitioning (histograms) with stratified sampling and extend it to handle dynamic updates efficiently. Multi-dimensional histograms usually cannot be updated easily under arbitrary insertions and deletions, for example \cite{thaper2002dynamic, gilbert2002fast} do not handle general updates, and \cite{donjerkovicdynamic} does not guarantee optimality. Furthermore, most histograms focus on equi-depth, equi-width or V-optimal partitioning.
We maintain a partitioning that guarantees that the confidence intervals we get are close to the optimum (shortest) confidence intervals we could have from the best partitioning. 
}

\reviewone{
In addition, mergeable summaries~\cite{agarwal2012mergeable, gan2020coopstore} focus mostly on frequency and quantiles problems.
Traditional mergeable summaries for aggregation queries mainly include (uniform, stratified, reservoir) sampling. While sampling techniques support efficient updates in the database, the error is far from optimum.
Our method is essentially a technique that uses mergeable summaries for aggregation queries. However, in contrast to traditional mergeable summaries, our new system uses a more involved technique: Maintain a partitioning over the space and a stratified sampling under arbitrary insertions and deletions. When we get a query we combine low-error (updated) summaries with only a few (updated) higher-error summaries to return a better estimation than traditional mergeable summaries techniques.
}

Thus, it is understood that most synopsis data structures have at least one of the following pitfalls in our desired dynamic setting: throughput, drift, or generality~\cite{chaudhuri2017approximate}.


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25]{figures/overview.png}
    \caption{\sys manages a collection of \syn synopses by maintaining them online while periodically re-optimizing partitioning and sample allocation. \label{fig:overview}}\vspace{-0.5em}
\end{figure}

This paper explores the DAQP problem and studies ways that we can mitigate the pitfalls of prior approaches with a flexible synopsis data structure that can continuously re-optimize itself.
We present \sys, a new DAQP system, which supports SUM, COUNT, AVG, MIN, and MAX queries with predicates under arbitrary insertions and deletions to the dataset. 
The main data structure in \sys is a dynamic extension of our recently published work~\cite{liang2020fast,liang2021combining}, which we call a Dynamic Partition Tree (\syn).
\syn is a two-layer synopsis structure that consists of a: (1) hierarchical partitioning of a dataset into a tree, and (2) a uniform sample of data for each of the leaf partitions (effectively a stratified sample over the leaves).
An optimizer determines the best partitioning conditions and sample allocations to meet a user's performance goals.
For each partition (nodes in the tree), we calculate the SUM, COUNT, MIN, and MAX values of the partition.
Any desired SUM, COUNT, AVG, MIN, and MAX query can be efficiently decomposed into two parts with the structure: a combination of the partial aggregates where the predicate fully covers a partition in the tree, and an approximate part where the predicate partially covers a leaf node (and can be estimated with a sample).
More importantly, this structure is essentially a collection of materialized views and samples, which can be maintained incrementally.

A core contribution of \sys is online synopsis optimization.
\sys continuously monitors the accuracy of all of its \syn synopses to account for data and workload drift. 
When a synopsis is no longer accurate, it triggers a re-optimization procedure that resamples and repartitions the data. 
This re-optimization problem is both a significant algorithmic and systems challenge.
From an algorithmic perspective, \sys needs an efficient way to determine the optimal partitioning conditions in dynamic data.
We propose an efficient algorithm based on a dynamic range tree index that finds a partitioning that controls the minimax query error (up to an approximation factor).
From a systems perspective,  re-optimization poses a bit of a logistical challenge.
New data will arrive as the new synopsis data structure is being constructed. We design an efficient multi-threaded catch-up processing algorithm that synchronizes new data and historical data without sacrificing the statistical rigor of the estimates. 

\reviewone{
Overall, the new system \sys we proposed has the following benefits over previously known indexes for approximate query processing. It handles arbitrary dynamic updates efficiently (comparing to the static indexes PASS~\cite{liang2021combining}, VecrdictDB~\cite{park2018verdictdb}, or some dynamic histograms~\cite{gilbert2002fast} that do not handle arbitrary updates), it provides theoretical guarantees on the confidence intervals (comparing to the machine learning based indexes such that DeepDB~\cite{hilprecht2019deepdb}), the query procedure accesses only a small synopsis of data and does not touch the original data set so the communication throughput is low (comparing to other tree-based indexes such as~\cite{joshi2008materialized, jurgens1998r}), and the estimation error is always low (comparing to traditional sketches~\cite{cormode2011synopses}, or histograms for aggregation queries)  without making any assumption about the spatial/value-domain distribution of the data (comparing to~\cite{lazaridis2001progressive}). Furthermore, our new system maintains the strongest theoretical guarantees on the error comparing to all the other known methods we discussed. In particular, the confidence intervals we get are close to the optimum confidence intervals we could have from the best partitioning.}
%We highlight all differences in the related work.}

==> DynamicPASS_ICDE FULLARXIV/maxVarUpdates.tex <==
\subsection{Maximum variance under updates}
\label{sec:updateVar}


\mparagraph{Minimizing the error}
\stavros{TODO}
Static PASS~\cite{hellerstein2008quantitative} tries to find a tree structure such that its leaf nodes define a partition over the samples $\samples$ to (approximately) minimize the length of the longest confidence interval. Equivalently, in PASS they are trying to find a partition that minimizes the maximum error.
The authors in~\cite{liang2021combining} argue that instead of looking over all possible queries to minimize the maximum error they focus on queries that lie completely inside one bucket. Indeed, the optimum partition considering only queries that lie completely inside a bucket has error at most $\sqrt{k}$ times more than the error over the optimum partition for COUNT/SUM queries. For AVG queries the error of the optimum partition considering queries completely inside buckets is the same with the maximum error considering every possible query.

In dynamic PASS we have the same goal: minimize the length of the longest confidence interval. As we discussed in previous sections the number of samples $H$ (catch-up phase) is going to be much larger than the number of samples in $\samples$. In particular the sampling rate of the catch-up phase in the end of the catch-up phase is usually significantly higher than the sampling rate of samples we store in dynamic PASS. Hence we expect that the error (variance) of nodes in $U_2$ will be much lower comparing to the error of the nodes in $U_1$ for a query $q$. So we focus on finding a partition that minimizes the longest confidence interval of any possible query considering only the error from the leaf nodes that partially intersect the query.
Similarly to~\cite{liang2021combining}, considering only queries completely inside a bucket gives a $\sqrt{k}$ approximation for COUNT/SUM queries and $1$-approximation (optimum) for AVG queries. For $1$D it gives a $\sqrt{2}$ approximation for COUNT/SUM queries.

Notice that when we study a query $q$ completely inside a leaf node $u$ we only care about the variance $$V(q)=m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2$$ if $q$ is a  COUNT/SUM query, or $$V(q)=\frac{1}{|q|^2}\left[m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2\right]$$ if $q$ is an AVG query. This is true because the weight $w_u$ and the denominator $m_u$ in the confidence interval is the same for every query in $u$. Hence, we can only focus on the variance of queries in a node to find the one with the longest confidence interval. 
In order to make sure that we return accurate estimators we require that each bucket contains a sufficiently large amount of samples, roughly $\Omega(\frac{1}{\alpha}\log m)$ samples, where $\alpha$ is the sampling rate of $\samples$.
If that holds, it is known from~\cite{liang2021combining} that with high probability the ratio $\frac{N_u}{m_u}$ for any possible leaf node $u$ will be within a constant factor from the ratio $N/m$, so it will be almost the same for any bucket we construct.
Furthermore, we study queries that contain at least $\delta m$ samples from each bucket that they partially intersect, for a small parameter $\delta<1$. Otherwise a query does not include many samples and we are not be able to return an accurate estimator along with a reasonable confidence interval. We note that these assumptions were also made by the authors in the static PASS~\cite{liang2020fast}.
Finally, we define the following notation that is useful in the next sections. For a rectangle $R$, let $\optVar(R)$ be the variance of the query with the maximum variance in $R$.



An important procedure of our algorithms is to be able to find what is the maximum error of a query that lies completely in a leaf node. We explain how to do it for the queries COUNT, SUM, AVG.
In particular, we describe a stronger result: We construct a dynamic data structure over a set of samples $\samples$ with efficient update time such that given a query rectangle, it returns an approximation of the variance of the query with the maximum variance in the query rectangle.
This result leads to very efficient dynamic algorithms for checking the maximum variance and re-constructing a new partition, as we will see in the next section.
As the authors in~\cite{liang2021combining} we use the notation $\maxVar$ for this procedure, i.e., $\maxVar(R)$ returns an approximation of the maximum variance of a query (COUNT, SUM, or AVG) in a rectangle $R$.

\mparagraph{COUNT queries}
For COUNT queries it is known~\cite{liang2021combining} that the query with the maximum variance in a rectangle $R$ contains exactly $|R\cap P|/2$ samples.
Hence, we construct a dynamic range tree~\cite{} $T$ over $\samples$ with space $O(m\log^d m)$. $T$ can be constructed in $O(m\log^d m)$ time and can be updated in $O(\log^d m)$ time. Given a query rectangle $R$, we run a binary search using $T$ to find two rectangles that contain $|R_i|/2$ items. The query runs in $O(\log^d m)$ time.

\mparagraph{SUM queries}
In ~\cite{liang2021combining} the authors showed that given a rectangle $R$ we can find a $\frac{1}{4}$-approximation of the variance of the query with the maximum variance inside $R$ by doing the following simple procedure: Find two non-intersecting rectangles $R_1, R_2$ such that $R_1\cup R_2=R$, and $|R_1\cap P|=|R_2\cap P|=|R\cap P|/2$. Then, they compare $\sum_{t\in R_1\cap P}t.a^2$ with $\sum_{t\in R_2\cap P}t.a^2$ and they return the variance of the rectangle with the largest sum of squares. The variance of this rectangle is a $\frac{1}{4}$-approximation of the maximum variance in $R$.
Range trees work for any aggregation function so we can also use them to compute the sum of the values squared in a rectangle or the variance of a rectangle.
Hence, we can use a dynamic range tree as we had in the COUNT case returning a $\frac{1}{4}$-approximation of the maximum variance. Notice that in this case we use the range tree for all procedures: i) finding two rectangles with the same number of samples ii) computing the sum of their squared values, and iii) compute the variance of a rectangle. This data structure has exactly the same complexities as in the COUNT case.

%As the authors in~\cite{liang2021combining} showed, we need $O(\log^{d-1} m)$ time to find an approximation of the maximum variance query in a bucket, using a range tree. Using a dynamic range tree~\cite{} for every bucket, we can achieve $O(\log^d m)$ update time for any insertion/deletion of a sample, and we can get a $1/4$-approximation of the maximum variance query.

\mparagraph{AVG queries}
The authors in~\cite{liang2021combining} proposed a way in the offline case to get an approximation on the maximum variance AVG query in a set of samples. In particular, their algorithm returns a $\frac{1}{4}$-approximation in $1$D, $\frac{1}{8}$-approximation in $2$D and $\frac{\delta^{1-1/d}}{2}$-approximation for $d>3$ and it runs in time superlinear . 
Unfortunately, their data structures cannot be efficiently extended to the dynamic case we are interested in (is not known how to achieve $\polylog m$ update time).
Here we propose a new dynamic data structure for finding an approximation of the maximum variance AVG query in a query rectangle efficiently. The new data structure we propose does not only handle updates efficiently, unlike the data structures in~\cite{liang2021combining}, but it also improves the approximation factor for any dimension $d$.
%All their algorithms can be made dynamic using dynamic data structures. Here, we briefly discuss their data structures and how they can be made dynamic. In the end we propose a new approximation dynamic algorithm with better approximation factor that works in any constant dimension $d$.




%In $1$D they use a search binary tree that stores the sum of squares of $\delta m$ consecutive samples in the leafs. In the inner nodes it stores the maximum such value that appear in the subtree of the inner node. The tree can be constructed in $O(m\log m)$ time and has $O(m)$ space. Given an interval the tree structure can return a $\frac{1}{4}$-approximation in $O(\log m)$ time. When we insert or delete a sample $t\in P$ we need to update the sums of the leafs that $t$ participates in and udpate the maximum values in the inner nodes. Notice that any sample participates in at most $O(\delta m)$ leaf nodes, hence this tree can be updated in $O(\delta m + \log m)$ time. We can easily modify this tree to return a $\frac{1}{8}$-approximation in $O(\log \frac{1}{\delta})$ time, with update time $O(\frac{1}{\delta})$. In $2$D, they only use a range tree, so we can use a dynamic range tree~\cite{} and handle insertion or deletions. This data structure has $O(m\log^d m)$ space, can be updated in $O(\log^{d} m)$ time, and returns a $\frac{1}{8}$-approximation of the maximum variance in a rectangle in $O(\log^{d+2} m)$ time. In higher dimensions, they propose a modified k-d tree where each leaf contains $\delta m$ samples. They return the rectangle that corresponds to the leaf node with the maximum sum of squares of the values, as the query with the maximum variance. Given a query rectangle, this procedure finds a $\frac{\delta^{1-1/d}}{2}$-approximation of the maximum variance in $O(\min\{\frac{1}{\delta}\log^d m, m\log m\})$ time. This k-d tree can be made dynamic~\cite{} having roughly the same complexities.

For a set of samples $\samples$ we construct a dynamic range tree $T'$. We also initialize an empty dynamic data structure $T$ that stores weighted rectangles. Given a query rectangle $R$, it returns the rectangle with the highest weight that lies completely inside $R$. For example $T$ can be a dynamic range tree in $2d$ dimensions storing each rectangle as a $2d$ point by creating a point from its two main opposite corners.
Notice that every $d$-th level node $u$ of $T'$ corresponds to a rectangle $R_u$.
If $|R_u\cap P|\leq \delta m$ then we add $R_u$ in $T$ with weight $S(R_u)=\sum_{t\in R_u\cap P}t.a^2$. If $\delta m\leq |R_u\cap P|\leq 2\delta m$ we split $R_u$ into two rectangles $R_{u_1}, R_{u_2}$ such that $R_{u_1}\cup R_{u_2}=R_u$ and $|R_{u_1}\cap P|=|R_{u_2}\cap P|=|R_u\cap P|/2$. We add $R_{u_1}, R_{u_2}$ in $T$ with weights $S(R_{u_1})=\sum_{t\in R_{u_1}\cap P}t.a^2$, $S(R_{u_2})=\sum_{t\in R_{u_2}\cap P}t.a^2$.
The tree $T'$ can be constructed in $O(m\log^d m)$ time and it has $O(m\log^d m)$ space. In $T$ we might insert $O(m\log^d m)$ rectangles so it has $O(m\log^{3d} m)$ space and can be constructed in $O(m\log^{3d} m)$ time. For any insertion or deletion of a sample in $\samples$, $T'$ can be updated in $O(\log^d m)$ time by modifying at most $O(\log^d m)$ nodes. For each modified node we update accordingly the corresponding rectangle in $T$ in $O(\log^{2d}m)$ time. Furthermore, after an update we traverse the $d$-th level of the tree from the updated leaf nodes to their roots inserting or removing rectangles from $T$ accordingly. In the full version of the paper we describe an amortized way to update $T$ efficiently that can be made worst case update by standard techniques~\cite{}.
Overall our data structure can be constructed in $O(\log^{3d} m)$ time, has $O(\log^{3d} m)$ space and can be updated in $O(\log^{3d+1} m)$ time.


%and a modified dynamic range tree $T$ as follows. Let $u$ be a node of $T$ and $w_1, w_2$ are its two children. If $|R_{w_1}\cap P|=|R_{w_2}\cap P|<\delta m$ and $|R_u\cap P|>\delta m$ then we stop the execution of $T$ in this branch of the tree and we create the two nodes $w_1, w_2$ containing exactly $\delta m$ samples by expanding their corresponding rectangles to contain more samples. Notice that a sample might belong in both $w_1, w_2$. In this way we have a dynamic range tree where in every leaf node (in any level of the range tree) it contains exactly $\delta m$ samples. It is not necessary to construct $T$ as a separate data structure from $T'$ since we can easily run all procedures by slightly changing the procedures on $T'$ with a $\polylog m$ overhead. However, we refer to $T$ as a separate data structure for simplicity. For each leaf node $u$ (over all levels) of $T$ we store $S.u=\sum_{t\in R_u\cap P}t.a^2$. Then for each inner node $u$ in the last ($d$-th) level of $T$ we store and maintain the maximum $S_w$ value among the leaf nodes $w$ with root the node $u$, i.e., $M.u=\max_{w\in leaf(u)}S_w$, where $leaf(u)$ is the set of leaf nodes of the tree rooted at node $u$. Our data structure (both trees $T, T'$) is constructed in $O(m\log^d m)$ time, has $O(m\log^d m)$ space, and can be updated in $O(\log^d m)$ time.

Given a query rectangle $R$ such that $R\cap P>2\delta m$ (as the authors in~\cite{liang2021combining} assume) we show how to return an approximation of the maximum variance query  efficiently.
We search $T$ using the query rectangle $R$ and we get a set of $O(\log^{2d} m)$ canonical nodes that contain all rectangles completely inside $R$. From the canonical subsets we get the rectangle $q'$ inside rectangle $R$ with the largest weight.
If $|q'\cap P|<\delta m$ then 
using $T'$ we run binary search over all dimensions until we find an expansion of $q'$ that contains exactly $\delta m$ samples. This can be done in $O(\log^{d+1} m)$ time. Without loss of generality assume that $q'$ is this rectangle. Using $T'$ we measure the variance of $q'$ in $R$ in $O(\log^d m)$. In the end we return the variance of $q'$ as the approximation of the maximum variance AVG query in the query rectangle $R$. The query procedure takes $O(\log^{2d} m)$ time.


%If $u$ is a leaf node of $T$ visited by the query procedure that partially intersects $R$ we do the following. From the definition $|R_u\cap P|=\delta m$ so $|R_u\cap R\cap P|\leq \delta m$. Assume that indeed the rectangle $R_u\cap R$ contains less than $\delta m$ samples. In this case we want to make sure that we create a rectangle containing exactly $\delta m$ samples inside $R$. Using $T'$ we run binary search over all dimensions until we find an expansion of the rectangle $R_u\cap R$ that contains exactly $\delta m$ samples inside $R$. Let $R_u'$ be this expanded rectangle. Using $T'$ we also get $\sum_{t\in R_u'\cap P} t.a^2$. In the end, without loss of generality the query procedure in $T$ finds a set of $O(\log^d m)$ (possibly overlapping) rectangles that cover $R$ and each of the rectangles containing $\delta m$ samples. Using the pre-computed values $M.u$ along with the values $\sum_{t\in R_u'\cap P} t.a^2$ we computed in the query procedure we return the rectangle with the largest sum of squared values. Let $q'$ be that rectangle. Using $T'$ we measure the variance of $q'$ in $O(\log^d m)$ time. In the end we return the variance of $q'$ as the approximation of the maximum variance AVG query in the query rectangle $R$. The query procedure takes $O(\log^{2d} m)$ time since there are $O(\log^d m)$ rectangles (leaf nodes of $T'$) that partially intersect $R$ and for each of them we need $O(\log^d m)$ to find new rectangles fully inside $R$ that contain $\delta m$ samples.

Next, we show that the variance we return is a good approximation of the real maximum variance in rectangle $R$.
\begin{lemma}
It holds that $V(q')\geq \frac{1}{4\log^d m}\optVar(R)$.
\end{lemma}
\begin{proof}
Let $q$ be the AVG query (a rectangle) with the maximum variance in $R$. It is known from~\cite{liang2021combining} that $q$ contains at most $2\delta m$ and at least $\delta m$ samples.
Since $|R\cap P|\geq 2\delta m$ we have that $$|R\cap P|\sum_{t\in q'\cap P}t.a^2-\left(\sum_{t\in q'\cap P}t.a\right)^2\geq \frac{|R\cap P|}{2}\sum_{t\in q'\cap P}t.a^2,$$
following from Lemma A.2 in~\cite{liang2021combining}.
Next, notice that a query procedure on $T'$ with the query range $q$ would give a set of $\log^d m$ canonical rectangles that cover $q$ where each of them contains at most $2\delta m$ samples. We note that for each of these canonical rectangles in $T'$ there are at most two rectangles in $T$ containing the same items. Let $X$ be the set of rectangles in $T$ corresponding to the canonical rectangles in $T'$. From its definition it holds that $|X|\leq 2\log^d m$. All of these rectangles in $X$ lie completely inside $R$ so the query procedure will consider them to find the rectangle with the largest weight.
Hence it holds that 
$$\sum_{t\in q'\cap P}t.a^2\geq \max_{x\in X}\sum_{t\in x\cap P} t.a^2\geq \frac{1}{2\log^d m}\sum_{t\in q\cap P}t.a^2.$$ Overall we have,
\begin{align*}
    V(q')&=\frac{1}{|q'\cap P|^2}\left[|R\cap P|\sum_{t\in q'\cap P}t.a^2-\left(\sum_{t\in q'\cap P}t.a\right)^2\right]\\
    &\geq \frac{1}{|q'\cap P|^2}\frac{|R\cap P|}{2}\sum_{t\in q'\cap P}t.a^2\\
    &\geq \frac{1}{|q'\cap P|^2}\frac{1}{4\log^d m}|R\cap P|\sum_{t\in q\cap P}t.a^2\\
    &\geq \frac{|q\cap P|^2}{|q'\cap P|^2}\frac{1}{4\log^d m}\frac{1}{|q\cap P|^2}\left[|R\cap P|\sum_{t\in q\cap P}t.a^2-\left(\sum_{t\in q\cap P}t.a\right)^2\right]\\
    &\geq \frac{1}{4\log^d m}\mathcal{V}(R)
\end{align*}
\end{proof}
In the full version we show that if $d=1$ we can modify the data structure so that it gives an approximation factor $4$ while having slightly better complexities with respect to the exponents of the $\log m$ factor.

Overall, given a set $P$ of $m$ points in $d$ dimensions we can construct a data structure of space $O(m\cdot \polylog (m))$ in $O(m\cdot \polylog (m))$ time with update time $O(\polylog (m))$ such that given a query rectangle it finds an approximation of the maximum variance COUNT, SUM or AVG query inside $R$ in $O(\polylog (m))$ time.

%We propose a new algorithm to find an approximation of the maximum variance in any constant dimension $d$. Instead of constructing a k-d tree we construct a dynamic range tree~\cite{} where each leaf node contains $\delta m$ samples. It might be possible that a sample belongs in two leaf nodes that are siblings in order to make sure that each leaf node has $\delta m$ samples. For each leaf node $u$ in the $d$-th level of the range tree we store and maintain the sum of squares of the values of the items in $u$. Then we store the leaf nodes in a max-heap with respect to the sum of squares we computed. This data structure can be constructed in $O(m\log^d m)$ time and it has $O(m\log^d m)$ space. For an insertion or deletion of a sample $p$ the range tree can be updated in $O(\log^d m)$ time~\cite{}, so at most $O(\log^d n)$ nodes of the tree might be modified or inserted. For each modified/inserted node we compute its sum and we update the max-heap. The max-heap can be updated in $O(\log n)$ time so in total the update time of our data structure is $O(\log^{d+1} n)$. In order to find an approximation of the maximum variance query we return the rectangle that corresponds to the leaf node with the largest sum of squares, i.e., the leaf node at the root of the max-heap. Such a rectangle contains $\delta m$ samples with the largest sum of squares over all other $d$-level leaf nodes. Let $q^*$ be the rectangle that corresponds to the query with the maximum variance. A standard range tree can find a partition of $q^*$ with $O(\log^d m)$ canonical nodes/rectangles. Since $|q^*|\leq 2\delta m$ it is not possible that a canonical node will contain any of the leaf nodes of our modified range tree. Hence, for each canonical node $u$ of $q^*$ in the standard range tree we can always find one leaf node in our modified range tree that completely covers $u$. Following the proof in~\cite{liang2021combining} we show that our algorithm returns a $\frac{1}{4\log^d m}$-approximation of the maximum variance query.

==> DynamicPASS_ICDE FULLARXIV/partition-old.tex <==
In order to achieve faster algorithms we propose new dynamic data structures for various sub-problems. Mainly, we propose an efficient dynamic data structures such that given a query rectangle, it returns (approximately) the maximum variance of a query completely inside the query rectangle. Using this data structure, we can achieve a very fast construction of $\PASStree$ in any dimension $d$.
For $d=1$ we manage to design a very efficient algorithm making an assumption on the aggregation values of the items. In particular we assume that the values of items are bounded by a polynomial on $N$, i.e. the total number of items in the full dataset. This is usually the case in real datasets so it is not a strong assumption and it is made in several papers~\cite{guha2006approximation} for constructing histograms with low error. %We notice that the assumption is not needed in higher dimensions.

We start by introducing some basic notation and by defining some basic notions. Then we describe our new dynamic data structures for finding maximum error queries.
We continue by presenting the partition algorithm for $d=1$ and the partition algorithm for any dimension $d>1$.
In the end of this section we show an algorithm to decide when re-partition is needed.





Let $u$ be a leaf node of $\PASStree$ and let $q$ be a query completely inside $R_u$. In this case notice that $w_u=1$ for all types of queries.
From Section~\ref{sec:estimators}, recall that the variance of any COUNT or SUM query completely inside $R_u$ has a factor $\frac{N_u^2}{m_u^2}$. This factor is the same in all queries inside $u$ so without loss of generality we can skip it from the variance definition (considering queries inside $R_u$).
Furthermore, notice that the confidence interval of any query inside $R_u$ has a factor $\frac{1}{m_u}$ which is also the same. Hence, the problem of finding the query with the largest confidence interval in $u$ is equivalent to the problem of finding the query $q$ in $u$ that maximizes the following function.
If $q$ is a COUNT or SUM query:
$V(q)=m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2$
and if $q$ is an AVG query:
$V(q)=\frac{1}{|q|^2}\left[m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2\right]$.


In order to make sure that we return accurate estimators we require that each bucket contains a sufficiently large amount of samples, roughly $\Omega(\frac{1}{\alpha}\log m)$ samples, where $\alpha$ is the sampling rate of $\samples$.
%If that holds, it is known from~\cite{liang2021combining} that with high probability the ratio $\frac{N_u}{m_u}$ for any possible leaf node $u$ will be within a constant factor from the ratio $N/m$, so it will be almost the same for any bucket we construct.
Furthermore, we study queries that contain at least $\delta m$ samples from each bucket that they partially intersect, for a small parameter $\delta<1$. Otherwise a query does not contain many samples in a leaf node and we are not be able to return an accurate estimator along with a provable confidence interval. We note that these assumptions were also made by the authors in the static PASS~\cite{liang2020fast}.
Finally, we define $\optVar(R)$ to be the variance of the query with the maximum variance in $R$.

==> DynamicPASS_ICDE FULLARXIV/partition.tex <==
\section{Optimal \syn Partitioning}
\label{sec:partAlg}
\newcommand{\poly}{\textrm{poly}}
We next describe a new dynamic partitioning algorithm designed for the dynamic setting.

\subsection{Preliminaries and Problem Setup}
\label{subsection:prelimandsetup}
The partitioning algorithm analyzes the pooled reservoir sample of data to determine how best to partition the dataset.
The goal of the partitioning algorithm is to find a partitioning such that the subsequent queries issued to the \syn have low-error. 
Surprisingly enough, the partitioning algorithm does not need an exact query workload to perform this optimization. 
It simply needs a focus aggregation function (e.g., SUM, COUNT, AVG) and finds a partitioning that minimizes the worst-case query error for sufficiently large predicates.
Given a set of $O(m)$ samples $S$, the goal is to construct a data structure that supports the following operations.
(i) Insert or delete a sample from $\samples$ efficiently, and (ii) when a partitioning request comes, it creates a near-optimum partition tree $\PASStree$ in $o(m)$ time.

Let $Q$ be a set of possible aggregate queries with a predicate. \reviewtwo{And, let $\Theta$ be the set of all \syn synopses with $k$ leaf nodes. Each $\syn$ consists of a hierarchical rectangular partitioning having $k$ partitions/buckets in the last level.} The main optimization we need to solve to find a good enough partitioning is to minimize the maximum error over the query workload:
\vspace{-0.8em}
\begin{equation}
    \min_{\PASStree \in \Theta} \max_{q \in Q} \textsf{Error}(q,\PASStree)
\end{equation}
The error is defined as the length of the confidence interval, as defined in the previous section. Since the catch-up variance is usually extremely smaller than the sample estimate variance, we focus on minimizing the maximum length of the confidence interval with respect to the sample estimate variance $\nu_s(\cdot)$.
\reviewone{Indeed, the catch-up phase is running in the background retrieving a large number of samples as the time passes. Hence, the estimations in every node of the \syn are constantly improving reducing $var(\phi_q(H_i))$ for each partition $R_i$. On the other hand, the number of samples $S$ that we are storing explicitly are limited making the sample estimate variance larger than the catch-up variance.}
For simplicity, when we say variance we always mean the sample estimate variance.
%As a proxy for this objective, one can minimize the maximum confidence interval length, which is equivalent to minimizing the maximum variance $\nu_s(q)$. 

Instead of looking over all possible queries to minimize the maximum error, one only needs to focus on single partitions to ensure they do not have ``high-variance'' sub-partitions (see Appendix~\ref{appndx:partAlg}).
Indeed by considering only these sub-partitions we can still get a $\sqrt{k}$-approximation for COUNT and SUM queries over the optimum partition considering all queries (for $k$ leaves). The approximation factor improves to $\sqrt{2}$ for $d=1$. For AVG queries the error of the optimum partition of this simplification is the same with the maximum error considering every possible query. 
The error of a query $q$ inside a leaf node (partition) $R_i$ is defined (expanding the equations from the definition of $\nu_s(\cdot)$) as
$$\frac{N_i^2}{m_i^3}\!\left[m_i\!\sum_{t\in q}\!t.a^2\!-\!\left(\!\sum_{t\in q}\!t.a\!\right)^2\right], \frac{m_i\!\sum_{t\in q}\!t.a^2\!-\!\left(\!\sum_{t\in q}\!t.a\!\right)^2}{m_i|q\cap \samples|^2}.$$
for SUM/COUNT and AVG queries, respectively.
Thus, the optimization problem reduces to finding partitions that do not contain a high-variance ``rectangle'' of data.


%In Subsection~\ref{sec:updateVar} we propose a new partitioning algorithm for $d=1$ that works in the dynamic case. In Subsection~\ref{sec:partHighDim} we design new indexes to extend the static algorithm from~\cite{liang2021combining}.

%We next show that a special indexing structure called a can be used for this purpose.
%The core procedure of our partitioning algorithm is to find what is the maximum error of a query that lies completely inside a rectangular region---once that can be done efficiently a simple search procedure can produce the partitioning condition.
%As one can imagine, these algorithms are straight-forward with provable guarantees in 1D (1 predicate attribute) and more heuristic in higher dimensions.

Given a rectangle $R$, the goal is to find a rectangular query within $R$ with maximum variance among all possible queries in $R\cap S$. For now, we assume that we have a dynamic index $\maxVar$ with near-linear space such that given a query rectangle $R$, it returns a query $q$ within $R$ with $\nu_s(q)\geq \frac{1}{\gamma}\optVar(R)$, \reviewone{for an approximation factor $\gamma>1$}, in $O(M)$ time, where $\optVar(R)$ is the variance of the maximum variance rectangular query in $R$. Let $\maxVar(R)$ be the variance of the query returned by the index $\maxVar$. We describe this index with more details in Subsection~\ref{sec:partHighDim}.

%One of the most common index we use in the next sections is the \emph{range tree}. A range tree~\cite{de1997computational} is a tree data structure that is built over a set of $n$ points in $\Re^d$ and it is used for aggregation or reporting rectangle range queries. Every point is stored in the leaf nodes and every inner node stores an interval defined over the maximum and the minimum coordinate of the points stored in the leaf nodes of the tree. Given a query rectangle, it returns the result of an aggregation query, such as a sum, in $O(\log^{d-1} n)$ time. The range tree can be made dynamic supporting insertions and deletions in $O(\log^d n)$ time~\cite{chan2017dynamic, mortensen2006fully}.



\subsection{Partitioning for $d=1$}
\label{subsection:1dpartitioning}
Now, we discuss how to solve the partitioning optimization problem in one dimension.
We present results for SUM and AVG queries. COUNT can be thought of as a special case of SUM with binary data.
The basic trick is to search over a discretized set of possible variance values.
For each value $e$, we try to construct a partitioning of $k$ partitions such that in each bucket the length of the longest confidence interval of a query is at most $e$.
By systematically reducing $e$ in each iteration, we control for the worst-case error.

%For COUNT queries the optimum partition in $1$D consists of equal size buckets (intervals) so we can find the new partition in $O(k\log m)$ time by maintaining $\samples$ in a dynamic search binary tree. Such a tree can be updated in $O(\log m)$ time while the order of the samples on the real line is the same as the order of the leaf nodes from left to right. When we have to (re-)construct the partition we find the right endpoint of each bucket using the search binary tree. Overall, we need $O(\log m)$ time to update the tree and $O(k\log m)$ time to construct a new partition.

\mparagraph{Bounding the Error}
The first step is to calculate the bounds for the maximum length of the largest possible confidence interval among queries that intersect one partition.
We assume that the aggregation value of any item in $\fullData$ is bounded by a maximum value $\mathcal{U}$ and a minimum non-zero value $\mathcal{L}$. We allow items to take zero values since this is often the case in real datasets but no item with positive value less than $\mathcal{L}$ or larger than $\mathcal{U}$ exists. We assume that $\mathcal{U}=O(\poly(N))$ and $\mathcal{L}=\Omega(1/\poly(N))$.
In Appendix~\ref{appndx:1dpartition}
we show that the length of the longest confidence interval is also bounded by $O(\poly(N))$ and $\Omega(1/\poly(N))$.
%In the full version of the paper~\cite{fullpaper} we show that the length of the longest confidence interval is also bounded by $O(\poly(N))$ and $\Omega(1/\poly(N))$.

%~\footnote{The proof is included in the full paper}

\forfullversion{
\begin{lemma}
\label{lem:bound}
Let $R$ be any rectangle and
let $\optVar_S(R), \optVar_A(R)>0$ be the variance of the SUM and AVG query respectively with the maximum variance in $R$. Then it holds that $\frac{\mathcal{L}}{\sqrt{2}}\leq \sqrt{\frac{\optVar_S(R)}{|R|}}\leq N\mathcal{U}$ and $\frac{\mathcal{L}}{\sqrt{2}N}\leq \sqrt{\frac{\optVar_A(R)}{|R|}}\leq \sqrt{N}\mathcal{U}$.
\end{lemma}
}
\forfullversion{
\begin{proof}
Without loss of generality let $q$ be the SUM or AVG query with the maximum variance in $R$.

First we focus on SUM queries. Let $N_R=|R\cap \fullData|$ be the number of total tuples in $R$. Unless $V(q)=0$, from~\cite{liang2021combining}, we know that there exists a query $q'$ with $|q'|=|R|/2$ such that $\frac{V(q)}{|R|}\geq \frac{N_R^2}{|R|^3}\frac{|R|}{2}\sum_{t\in q'}t.a^2$, where $\sum_{t\in q'}t.a^2>0$. We also have $\sum_{t\in q'}t.a^2\geq \mathcal{L}^2$ and $w_u=1$ leading to $\sqrt{w_u\frac{\optVar_S(R)}{|R|}}\geq\frac{N_R}{\sqrt{2}|R|}\mathcal{L}\geq \frac{\mathcal{L}}{\sqrt{2}}$. Furthermore, we have $V(q)\leq\frac{N_R^2}{|R|^2}|R|^2\mathcal{U}^2\leq N^2\mathcal{U}^2$ leading to $\sqrt{w_u\frac{\optVar_S(R)}{|R|}}\leq N\mathcal{U}$.

Next, we consider AVG queries. Unless $V(q)=0$, from~\cite{liang2021combining}, we know that there exists a query $q'$ with $|q'|=\delta m\leq |R|/2$ such that $\frac{V(q')}{|R|}\geq \frac{1}{|R|\delta^2m^2}\frac{|R|}{2}\sum_{t\in q'}t.a^2$, where $\sum_{t\in q'}t.a^2>0$. We also have $\sum_{t\in q'}t.a^2\geq \mathcal{L}^2$ and $w_u=1$ leading to
$\sqrt{w_u\frac{\optVar_A(R)}{|R|}}\geq \frac{1}{\sqrt{2}\delta m}\mathcal{L} \geq \frac{\mathcal{L}}{\sqrt{2}N}$.
Furthermore, we have $V(q)\leq\frac{|R|}{|q|^2}\mathcal{U}^2\leq |R| \mathcal{U}^2\leq N \mathcal{H}^2$ leading to $\sqrt{w_u\frac{\optVar_A(R)}{|R|}}\leq \sqrt{N}\mathcal{U}$.
\end{proof}
}
%Since, $\mathcal{U}, \mathcal{L}$ are bounded by a polynomial with respect to $N$, we have that the length of the longest confidence interval is also bounded by $O(\poly(N))$ and $\Omega(1/\poly(N))$.

%Since, $\mathcal{U}, \mathcal{L}$ are bounded by a polynomial with respect to $N$, we have that the length of the longest confidence interval is bounded by $O(\poly(N))$ and $\Omega(1/\poly(N))$, i.e. $$\Omega(1/\poly(N))\leq \sqrt{w_u\frac{\optVar_S(R)}{|R|}}, \sqrt{w_u\frac{\optVar_A(R)}{|R|}} \leq O(\poly(N)).$$

\mparagraph{Description of Algorithm}
We describe the partitioning algorithm for SUM queries. The procedure is identical for AVG queries.
For a parameter $\rho\in \mathbb{R}$ with $\rho>1$, let $E=\{\rho^t\mid t\in  \mathbb{Z}, \frac{\mathcal{L}}{\sqrt{2}}\leq \rho^t\leq N\mathcal{U}\}\cup\{0\}$, be the discretization of the %range $[\frac{\mathcal{L}}{\sqrt{2}}, N\mathcal{U}]$, i.e.,
range defined by
the lower and upper bound of the longest confidence interval (as defined in the previous paragraph).
%For an interval $b$, let $\MAXV(b)$ be the approximation of the query with the maximum variance in bucket $b$ (supporting updates) as described in Section~\ref{sec:updateVar}.
We run a binary search on the values of $E$. For each value $e\in E$ we consider, we try to construct a partitioning of $k$ partitions such that in each partition the length of the longest confidence interval of a query is at most $e$. If there exists such a partitioning we continue the binary search with values $e'<e$. If there is no such a partitioning we continue the binary search with values $e'>e$. In the end, we return the last partitioning that we were able to compute.

It remains to describe how to check if a partitioning with $k$ buckets (intervals) with maximum length confidence interval at most $e$ exists.
A high level description of the algorithm is:
\begin{enumerate}
    \item For $i=1$ to $k$
    \begin{enumerate}
        \item Let $b_i$ be the $i$-th bucket with left endpoint
    $t_a$
        \item Binary search on samples $t_j$ to find the maximum bucket $b_i$ with error at most $e$
        \item If $\sqrt{\maxVar([t_a, t_j])}\leq e$
        \begin{enumerate}
            \item Continue search for values $>j$
            \item Else Continue search for values $<j$
        \end{enumerate}
    \end{enumerate}
    \item If the partitioning contains all samples construct $\PASStree$ using $b_i$ as its leaf nodes. Otherwise $\PASStree=\emptyset$.
\end{enumerate}
We start with the leftmost sample, say $t_1$, which is the left boundary of the first bucket. In order to find its right boundary we run a binary search on the samples $\samples$. Let $t_j$ be one of the right boundaries we check in the binary search, and let $b_1=[t_1, t_j]$. If $\sqrt{\MAXV(b_1)}\leq e$ then we continue the binary search with a sample at the right side of $t_j$ (larger bucket). Otherwise, we continue the binary search with a sample at the left side of $t_j$ (smaller bucket). When we find the maximal bucket with longest confidence interval at most $e$ we continue with the second bucket repeating the same process for at most $k$ buckets. In the end, if all samples in $\samples$ are contained in $k$ buckets then we return that there exists a partitioning (with $k$ buckets) with maximum variance at most $e$. If we cannot cover all samples in $k$ buckets then we return that there is no partitioning with $k$ buckets and maximum variance at most $e$.
%We skip a corner case from the description of the algorithm where the partitioning of maximum error $e$ exists but the last $k$-th partition contains a small number of samples from $\samples$. We can handle this case by storing two intersecting leaf nodes in $\PASStree$ and handling it carefully having exactly the same guarantees.



\forfullversion{
\SetKwComment{Comment}{/* }{ */}
\begin{algorithm}
\caption{}\label{alg:one}
\KwData{$e, \samples, k, \eta$}
\KwResult{$\PASStree$}
$j \gets 0$\;
\For{$i=1$ to $k$}{
    $i_1\gets j+1$, $i_2\gets |\samples|-1$\;
    \uIf{$i_1>|\samples|$}{
        \textbf{break}\;
    }
    \While{$i_1\leq i_2$}{
        $i_3\gets \text{floor}((i_1+i_2)/2)$\;
        \uIf{$i_3-i_2+1\geq \eta$}{
            $W\gets \maxVar([t_a,t_{i_3}])$\;
            \uIf{$\sqrt{\frac{W}{i_3-i_2+1}}\leq e$}{
                $j\gets i_3$\;
                $i_1\gets i_3+1$\;
            }\Else{
                $i_2\gets i_3-1$\;
            }
        }\Else{
            $i_1\gets i_3+1$\;
        }
    }
    $b_i\gets [t_a, t_j]$\;
}
\uIf{$\left(\bigcup_i b_i\right)\cap \samples =\samples$}{
    Construct search binary tree $\PASStree$ using $b_i$ as leaf nodes\;
    \Return $\PASStree$\;
}\Else{
    $\PASStree\gets \emptyset$\;
}
\end{algorithm}
}


%The same algorithm also works for AVG queries. The only difference is that $E$ should be defined with respect to the upper and lower bound of the longest confidence interval, as shown in Lemma~\ref{lem:bound}.

\textbf{Correctness. }
In Appendix~\ref{appndx:1dpartition} we use the monotonic property of the longest confidence interval (the bigger the bucket the larger the error) and we show $\sqrt{\optVar(b')}\leq \sqrt{\gamma \MAXV(b')}\leq \sqrt{\gamma} e'\leq \rho\sqrt{\gamma} \sqrt{\optVar(b^*)}$, where $b'$ is the bucket with the longest confidence interval in the returned partitioning, $e'$ is the smallest value in $E$ such that $\sqrt{\optVar(b^*)}\leq e'$, and $b^*$ is the bucket of optimum partitioning with the largest confidence interval.
For $d=1$ we have that $\gamma=4$ for SUM and AVG queries queries, so we get a partitioning where the maximum error is within $2\rho\sqrt{2}$ of the optimum error for SUM queries and within $2\rho$ of the optimum error for AVG queries.

%Before we start with the correctness proof of our algorithm we recall that in~\cite{liang2021combining} we showed that under a mild assumption, for two buckets $b_i, b_j$ if $b_i\subseteq b_j$ then $\sqrt{\optVar(b_i)}\leq \sqrt{\optVar(b_j)}$, namely the length of the longest confidence interval in $b_i$ is smaller than the length of the longest confidence interval in $b_j$. We call it the monotonic property of the longest confidence interval.


%Let $\mathcal{R}^*$ be the optimum partitioning and let $b^*$ be the bucket that contains the query with the longest confidence interval in $\mathcal{R}^*$. First, we notice that if $e\geq \sqrt{\optVar(b^*)}$ then we always find a partitioning with longest confidence interval at most $e$. We can show it by induction on the right boundaries of the buckets (intervals) and the monotonic property of confidence intervals. We show all details in the full version of the paper.
\forfullversion{
For the base case,  let $b_1^*=[t_1, t_2]$ be the first bucket of partitioning $\mathcal{R}^*$. The procedure $\MAXV$ always underestimates the maximum variance in an interval so the binary search in our procedure will consider the right boundary to be greater than $t_2$.
Let $t_i$ be the right boundary of the $i$-th bucket in $\mathcal{R}^*$ and let assume that the $i$-th bucket in our procedure has a right boundary $t_j\geq t_i$.
We consider the $(i+1)$-th bucket in $\mathcal{R}^*$ with boundaries $[t_{i+1}, t_r]$. We show that the $(i+1)$-th bucket in our procedure has a right boundary at least $t_r$. Let $[t_a, t_b]$ be the boundaries of the $(i+1)$-th bucket in our procedure. We have $t_a\geq t_{i+1}$. If $t_a=t_{i+1}$ then $t_b\geq t_r$ as in the basis case. If $t_a>t_{i+1}$ then because of the monotonic property of the confidence intervals and the fact that the $\MAXV$ procedure underestimates the maximum variance we also have that $t_b\geq t_r$.
}
%Let $e'$ be the smallest value in $E$ such that $\sqrt{\optVar(b^*)}\leq e'$. Because of the previous observation our algorithm always returns at least a valid partitioning for an $e\leq e'$. For every bucket $b$ of this partitioning, $\sqrt{\MAXV(b)}\leq e$. Let $b'$ be the bucket in the returned partitioning containing the query with the longest confidence interval. We have, $\sqrt{\optVar(b')}\leq \sqrt{\gamma \MAXV(b')}\leq \sqrt{\gamma} e\leq \sqrt{\gamma} e'\leq \rho\sqrt{\gamma} \sqrt{\optVar(b^*)}$.

%From Appendix~\ref{sec:updateVar} we have that $\gamma=4$ for SUM and AVG queries queries. So we get a partition where the maximum error is within $2\rho\sqrt{2}$ of the optimum error for SUM queries and within $2\rho$ of the optimum error for AVG queries.

\textbf{Running time. }
%We assume that $\MAXV(\cdot)$ can be computed in $M$ time.
Since, $\mathcal{L}, \mathcal{U}$ are polynomially bounded on $N$ we have that $|E|=O(\log_\rho N)$ and it can be constructed in $O(\log_\rho N)$ time. The binary search over $E$ takes at most $O(\log \log_\rho N)$ steps.
%For each value $e\in E$ of the binary search we check if there is a partitioning with $k$ buckets and longest confidence interval at most $e$. For each possible bucket we run a binary search over the samples $\samples$ and we run the procedure $\MAXV$ to get an approximation of the maximum variance.
We can decide if there exists a partitioning with error $e$ in $O(kM\log m)$ time. Overall, the running time of our algorithm is $O(kM\log m \log\log_\rho N)$. If $\rho$ is a constant, for example $\rho=2$, then the running time is $O(kM\log m \log\log N)$. In Appendix~\ref{appndx:partAlg}
%From Appendix~\ref{sec:updateVar}
we have that in $1$-dimension $M=O(\log m)$ for SUM and AVG queries. Notice that if we skip the $\log$ factors the running time depends only linearly on the number of buckets $k$ and the approximation factor is constant.

\subsection{Partitioning in Higher Dimensions}
\label{sec:partHighDim}


\subsubsection{Indexing To Find Maximum Variance}\label{sec:NewupdateVar}
We describe the core index $\maxVar$ that we use in all our partitioning algorithms for any dimension $d\geq 1$. All the details and technical proofs will be shown in Appendix~\ref{sec:updateVar}.
The exact description of the index depends on the type of aggregation queries we focus on. %However, in all cases we construct a specific modified dynamic range tree.

For SUM/COUNT queries,
%using the results in ~\cite{liang2021combining}
we propose a simple index to find the query with the largest variance in a query rectangle. In particular, we build a dynamic range tree on $\samples$. Given a query rectangle $R$, we split it into two smaller rectangles $R_1, R_2$ such that $|R_1\cap \samples|=|R_2\cap \samples|=|R\cap \samples|/2$. Using a dynamic range tree~\cite{de1997computational} we return the rectangle $R_i$ (either $R_1$ or $R_2$) with the largest variance. We can show that $\nu_s(R_i)\geq \frac{1}{4}\optVar(R)$. The running time and the update time is $O(\log^d m)$. 

For AVG queries, the algorithm proposed in~\cite{liang2021combining} cannot be extended to the dynamic case. Hence we propose a new dynamic index with a better approximation factor. Similarly to ~\cite{liang2021combining}, we assume that every valid query that is contained in a bucket of the partitioning must contain at least $2\delta m$ samples (for a small parameter $\delta<1$), otherwise the estimation is not accurate.
For simplicity, we use the notation $\tilde{O}(\cdot)$ to hide $\log(m)$ factors.
In Appendix~\ref{sec:updateVar} we show the following crucial observation: for any rectangle $q$ inside a query rectangle $R$ with $|q\cap \samples|=\delta m$ that maximizes $\sum_{t\in q\cap \samples} t.a^2$, it holds that $\nu_s(q)\geq \frac{1}{4}\optVar(R)$. Hence, we build a dynamic index
%(in particular our index consists of two dynamic range trees), 
so that given a query rectangle $R$ it returns a rectangle that contains $\delta m$ samples and the sum of squares of their aggregate values is close to the maximum sum.

We build a dynamic range tree $T'$ over the samples $\samples$, storing the number of samples in each node of the tree. %with respect to the sum of their values or the sum of their square values. 
Furthermore, we build another empty dynamic range tree $T$. We will use $T$ to store weighted rectangles (as points in $2d$) that contain at most $\delta m$ samples. More specifically, we store in $T$ the \emph{canonical} rectangles of $T'$ that contain at most $\delta m$ samples. Notice that there are $\tilde{O}(m)$ nodes in $T'$ hence $T$ uses $\tilde{O}(m)$ space.
When we have an insertion or deletion in $T'$ there are only $\tilde{O}(1)$ nodes/rectangles that are updated, hence we can update both $T'$ and $T$ in $\tilde{O}(1)$ time.
Given a query rectangle $R$ we use $T$ to find a rectangular query $q^*$ with the largest sum inside $R$ in $\tilde{O}(1)$ time. From the definition of a range tree, for any rectangle there is a partitioning of $\log^{d+1} m$ canonical rectangles from $T'$. Hence we can show that $\nu_s(q^*)\geq \frac{1}{4\log^{d+1} m}\optVar(R)$.
The exact complexities depend on the dynamic range tree structure we use; our data structure has roughly $O(m\log^{3d} m)$ space, $O(\log^{3d} m)$ update time, and $O(\log^{2d} m)$ query time.


%More specifically, we build a dynamic range tree $T'$ over the samples $\samples$, storing the number of samples in each node of the tree. %with respect to the sum of their values or the sum of their square values. Furthermore, we build another empty dynamic range tree $T$. We will use $T$ to store weighted rectangles (as points in $2d$) that contain at most $\delta m$ samples. Each node $u$ of $T'$ is associated with a rectangle $R_u$. If $|R_u\cap \samples|\leq \delta m$ then we add $R_u$ in $T$ with weight $\sum_{t\in R_u\cap S}t.a^2$. If $\delta m<|R_u\cap \samples|\leq 2\delta m$ then we split $R_u$ into two rectangles $R^1_u, R^2_u$ with cardinality $|R_u\cap \samples|/2$ and we add $R_u^1, R_u^2$ in $T$ with weights $\sum_{t\in R^1_u\cap \samples}t.a^2$ and $\sum_{t\in R^2_u\cap \samples }t.a^2$, respectively. Notice that there are $\tilde{O}(m)$ nodes in $T'$ hence $T$ uses $\tilde{O}(m)$ space. When we have an insertion or deletion in $T'$ there are only $\tilde{O}(1)$ nodes/rectangles that are updated (either their structure or the stored counts), hence we can update both $T'$ and $T$ in $\tilde{O}(1)$ time. Given a query rectangle $R$ we use $T$ to find a rectangular query $q^*$ with the largest sum inside $R$ in $\tilde{O}(1)$ time (if the rectangle we find has less than $\delta m$ items we arbitrarily extend the rectangle inside $R$ to contain exactly $\delta m$ samples). Notice that for any rectangle there is a partition of $\log^{d+1} m$ canonical rectangles from $T'$. Hence we can show that $\nu_s(q^*)\geq \frac{1}{4\log^{d+1} m}\optVar(R)$. The exact complexities depend on the dynamic range tree structure we use, however our data structure has roughly $O(m\log^{3d} m)$ space, $O(\log^{3d} m)$ update time, and $O(\log^{2d} m)$ query time.

%The overall data structure for our variance calculation is a modified dynamic range tree. We note that any variance can essentially be represented as the difference of two sums: sum of squares and the square of the sum.
%For particular focus functions, the technical details differ.
%In particular, for COUNT queries we construct a data structure of $O(m\log^d m)$ space that can be updated in $O(\log^d m)$ time such that given a query rectangle it finds the maximum variance query in $O(\log^d m)$ time.
%For SUM queries we construct a data structure with the same guarantees as in the COUNT data structure but it returns a $\frac{1}{4}$-approximation of the maximum variance. For AVG queries we construct a data structure of $O(m\log^{3d} m)$ space that can be updated in $O(\log^{3d+1} m)$ time such that given a query rectangle it finds a $\frac{1}{4\log^{d+1} m}$-approximation of the the maximum variance query in $O(\log^{2d+1} m)$ time.
%In the next subsections we use the notation $\maxVar(R)$ for the value of the variance returned by our approximation algorithm in a rectangle $R$.


\subsubsection{Partitioning}
%We assume that $\MAXV$ returns a $\frac{1}{\alpha}$-approximation in $M$ time.
We construct a partitioning by building a k-d tree using the dynamic procedure $\MAXV$ as we described above.
Here, we use our improved index $\maxVar$ to construct a k-d tree.
The high level description of the algorithm is:
\begin{enumerate}
    \item Max Heap $C$ containing partition $R_1$ covering all items in $\fullData$
    \item For $j=2$ to $k$
        \begin{enumerate}
            \item Extract partition $R_i$ with maximum $\maxVar(R_i)$ from $C$
            \item Create a partitioning of $R_i$ of two partitions $R_{i_1}$, $R_{i_2}$ by splitting on the median of $R_i$
            \item Insert $\maxVar(R_{i_1})$, $\maxVar(R_{i_2})$ in $C$
            \item Set $R_{i_1}$, $R_{i_2}$ as children of $R_i$ in $\PASStree$
        \end{enumerate}
\end{enumerate}
%We start by constructing a dynamic data structure from Section~\ref{sec:updateVar} over the initial set of samples $\samples$.
%Assume that after a number of updates in $\samples$ we want to (re)construct the tree structure $\PASStree$ over $\samples$.
%We pre-define an ordering of the dimensions.
%Each node $i$ of the tree is associated with a partition/rectangle $R_i$.
%We build the tree in $k$ iterations in a top-down manner starting from the root which is associated with a partition $R_1$ such that $\fullData\subset R_1$. 
%In any iteration we store and maintain the approximate maximum variance queries of every leaf node in a max heap $C$. In the end of the $j$-th iteration we have a tree of $j$ leaf nodes. Let $R_i$ be the partition of the leaf node with the maximum $\maxVar(R_i)$ value in $C$. We remove its value from $C$. We find the medium coordinate with respect to the next dimension in the ordering (in this branch of the tree) among the samples $R_i\cap \samples$. We split $R_i$ on the median into two partitions $R_{i_1}, R_{i_2}$ and we add them as children to the node of $R_i$. Using the algorithms from Section~\ref{sec:updateVar} we compute $\maxVar(R_{i_1}), \maxVar(R_{i_2})$ and we insert their values in the max-heap $C$. We continue with the same way until we construct a tree $\PASStree$ with $k$ leaf nodes (buckets).


We can show that such a tree construction returns a partitioning which is near optimal with respect to the optimum partition tree construction following the same splitting criterion: split on the median of the leaf node with the largest maximum variance query. %In our case we do not always split the nod with the real largest error since we use the approximation function $\maxVar(\cdot)$.
Overall we construct a data structure that can be updated in $O(\polylog m)$ time.
For a (re-)partition activation over a set $\samples$ of $m$ samples, we can construct a new $\PASStree$ with the following guarantees: For COUNT/SUM queries, $\PASStree$ can be constructed in $O(k\log^d m)$ time with approximation factor $2\sqrt{k}$.
%For COUNT queries we get the same construction time $O(k\log^d m)$ but the tree we construct is optimum (with respect to the partition tree with same split criterion).
For AVG queries, $\PASStree$ can be constructed in $O(k\log^{2d} m)$ time with approximation factor $2\log^{(d+1)/2} m$.
%In all cases we can construct near-optimum partitions in $\tilde{O}(k)$ time.

%We also propose a new heuristic to construct the k-d tree. In some cases it might not be a good idea to split always at the median. Ideally, we want to split at the best \emph{separator}, i.e., find the axis parallel hyperplane that splits a node into two nodes with the minimum largest variance. Assume a node $u$ of the k-d tree. Let $u$ be a node of the k-d tree that we decided to split (because it has the largest maximum variance comparing to the other current leaf nodes). We consider all possible axis parallel hyperplanes and we choose the one such that $\max\{V(u_1), V(u_2)\}$ is the minimum among all the other hyperplanes, where $u_1, u_2$ are the children of node $u$. We still use the $\MAXV$ function to get an approximation of the maximum variance in each possible hyperplane. If there are $O(m)$ samples in a node then there are $O(m)$ possible axis parallel separators that we need to check. Hence, the running time would be $O(msk)$, skipping the $\log m$ factors. Instead, we implement this algorithm more efficiently. Because of the the monotonic property of the maximum variance, for each dimension $i$ we can run a binary search on the hyperplanes perpendicular to dimension $i$ until we find the hyperplane with the smallest maximum variance. Indeed, by trying perpendicular hyperplanes from smaller to larger values, we are increasing the maximum variance in one bucket and we are decreasing the maximum variance in the other bucket. Hence a binary search will find the hyperplane that (approximately) minimizes the maximum variance in both buckets. We repeat the same for every dimension and we keep the separator/hyperplane that gives the children with the smallest maximum variance query. If $\MAXV$ takes $s$ time this will return a partition of $k$ buckets in $O(ks\log^{d+2} m)$ time.

\subsection{Re-Partitioning Triggers}
\label{sec:re-partition}
Assume that the current partitioning is $\mathcal{R}$ and let $\maxVar(\mathcal{R})$ be the (approximate) maximum variance query with respect to the current set of samples $\samples$.
\sys first checks the number of samples in each bucket (leaf node) of the current $\PASStree$. If there is a leaf node $i$ associated with partition $R_i$ such that $|\samples_i|<<\frac{1}{\alpha}\log m$ (where $\alpha$ is the sampling rate) then there are not enough samples in $u$ to make robust estimators. Hence, we need to find a new re-partitioning. Even if the number of samples in each bucket is large our system might enable a re-partitioning:
For a partition $R_i$ in the leaf node layer of $\PASStree$ let $\maxVar_i=\maxVar(R_i)$ be the (approximate) maximum variance at the moment we constructed $\PASStree$. Let $\beta>1$ be a parameter that controls the maximum allowable change on the variance. It can either be decided by the user or we can set it to $\beta=10$. Assume that an update occurred in the leaf node associated with the partition $R_i$. After the update we get $\maxVar_i'=\MAXVar(R_i)$. %and we update $\maxVar(\mathcal{R})$ if needed.
If $\frac{1}{\beta}\maxVar_i\leq \MAXVar_i'\leq \beta\MAXVar_i$ then the new maximum variance in partition $b_i$ is not very different than before so we do not trigger a re-partition. Otherwise, the maximum variance in bucket $b_i$ changed by a factor larger than $\beta$ from the initial variance $\maxVar_i$.
In this case a re-partitioning might find a new tree with smaller maximum error.
%Using the algorithms from the previous subsections we compute a new partitioning $\mathcal{R}'$ and hence a new tree $\PASStree$.
We compute a new partitioning $\mathcal{R}'$ and hence a new tree $\PASStree$.
If $\maxVar(\mathcal{R}')<\frac{1}{\beta}\maxVar(\mathcal{R})$ then we activate a re-partition restarting the catch-up phase over the new tree $\PASStree$. On the other hand, if $\maxVar(\mathcal{R}')\geq \frac{1}{\beta}\maxVar(\mathcal{R})$ then our current partitioning $\mathcal{R}$ is good enough so we can still use it.
%Our algorithm can decide if a re-partitioning is needed in $O(\polylog(m))$ time or $O(\polylog (m) +k)$ in the worst case.
Of course, the user can also manually trigger re-partitioning. For example, the user can choose to re-partition once every hour, day, or after $\tau$ insertions and deletions have occurred. In Appendix~\ref{appx:re-partition}, we also describe how \sys can execute either partial or full re-partitioning.

\iffalse
\sys can either apply entire or partial re-partitioning when is needed. Entire re-partitioning is straightforward as we described in the previous sections. For partial re-partitioning we only re-construct the tree around the area of the ``problematic'' leaf node using our dynamic procedures. Due to space limits we describe this procedure with more details in the full version of the paper.
Generally, the error of queries after a partial re-partitioning is lower than the error of the queries immediately after an entire re-partitioning. This is because entire re-partitioning needs to compute from scratch all estimations in the catch-up phase while the partial re-partitioning can still use the accurate estimators in the nodes that have not been changed.
However, in both cases we need to restart the catch-up phase over the new tree in order to get good estimators to the nodes that were changed by the re-partitioning.
\fi

%Next, we propose two ways to re-partition the index. In particular, the user can select either partial re-partitioning or entire re-partitioning. Entire re-partitioning is easy; using the algorithms from the previous subsections we can construct a new partitioning and a new tree structure in near-linear time with respect to the samples. Hence, we focus on partial re-partitioning. Instead of re-partitioning the entire space we can only re-partition the area around the "problematic" leaf node. Let $b_i$ be this leaf node with high error or small number of samples. In order to define the neighboring area around $b_i$ we propose either a predefined way or an automatic way. In both cases, the neighboring area is defined by a parameter $\psi$, which is the level of the tree above $b_i$ that the tree needs to be updated. In the predefined way, the parameter $\psi$ is a known parameter. We find the node $v$ which is defined as an ancestor of the leaf node $b_i$, $\psi$ levels above $b_i$. Let $\PASStree_u$ is the subtree with root node $u$ and let $l_u$ be the number of leaf nodes in $\PASStree_u$. Using the algorithms from the previous subsections we find a near optimum partition starting from node $u$ with $l_u$ leaf nodes. The running time is near-linear with respect to the samples stored $\PASStree_u$. In the automatic way, we do not know the parameter $\psi$ upfront so we try different values of $\psi$ running a binary search on the levels of the tree until we find a partition with low enough error. For each different value of $\psi$ we try, we run the same partial re-partitioning algorithm as in the static case starting from the node $u$ we are considering in the binary search.
%Notice that if the automatic partial re-partitioning does not find a good enough partitioning, it might reconstruct the entire tree.
%In the worst case the running time of the automatic partial partitioning is $\tilde{O}(m\log (\text{height}(\PASStree)))$, however in practice it usually runs much faster than the entire re-partitioning.

%Generally, partial re-partitioning is faster than the entire re-partitioning since it only suffices to find a better partitioning in a small area of the space. Furthermore, in partial re-partitioning we can still keep all the current estimations in all nodes of $\PASStree\setminus \PASStree_u$, i.e., the nodes of the tree that are not changed. Hence, the error of queries after a partial re-partitioning is also lower than the error of the queries immediately after an entire re-partitioning. However, in both cases we need to restart the catch-up phase over the new tree in order to get good estimators to the nodes that were changed by the partial re-partitioning.
%Recall that we cannot get samples from a particular area (ideally samples that stored in the leaf nodes of $\PASStree_u$) hence we run the catch-up phase getting samples from the entire space. We finally note that while the catch-up phase considers samples from the entire space, we only use these samples to improve the estimators in the nodes that are still under-represented, i.e., the catch-up phase time threshold for these nodes has not been completed.



\reviewtwo{
\subsection{Discussion: Selection of Parameters and Single Synopsis}
\label{subsection:discussion}
}
\newchanges{
Given a memory constraint, our system defines the parameters $m, k$, i.e. the number of samples and the number of leaf nodes in \syn. The asymptotic space of our index, as we saw in the previous subsections, is roughly $O(m+k)$, skipping $\log m$ factors. However, $k\ll m$ so the asymptotic space of our system is $O(m)$. In particular, in our experiments we observed that choosing $k\approx \frac{0.5}{100}m$ always gives a low space and efficient data structure with low error guarantees.
%A similar bound was observed in~\cite{liang2021combining}.
Hence, using the memory constraint, the space of our index with respect to $m, k$, and the relation between $m, k$ our system can automatically set these parameters.
If the user also gives a query processing constraint, we might change the values of $m, k$ to satisfy this requirement. In particular, the query time of our index is $O(k+\min\{\log^d m, m^*\})$, where $m^*$ is the maximum number of samples in a leaf node, which is typically no more than $2\cdot m/k$.  
}


\reviewtwo{
So far, we consider that the user defines different synopses for different query templates.
We recall that for a query template the user should give three inputs: i) the type of the query SUM/COUNT/AVG/MAX/MIN, ii)the aggregation attribute $A$, and iii) the predicate attributes $c_1,\ldots, c_d$. Any combination of these inputs creates a different template.
We propose two ways to handle multiple templates. The first one has the same theoretical guarantees with respect to the maximum confidence interval as we had for a single synopsis.
In the second one, we present a simpler heuristic way to handle multiple query templates. We can still have confidence intervals but we do not have any guarantee over them.
%on how far the confidence intervals are with respect to the optimum confidence intervals we could get from an optimum partitioning.
}

\reviewtwo{
First method: Recall that a synopsis consists of the partition tree \syn and a set of at most $2m$ samples $\samples$. As we described previously the overall space for a synopsis is roughly $O(m+k)=O(m)$.
We describe a simple method having one global set $\samples$ of at most $2m$ samples and for each query template we only need to construct a different partition tree \syn. Hence, if the user is interested in $L$ different query templates the total space of our index is $O(m+L\cdot k)$.
The main idea is that we store $\samples$ only once in a dynamic range-tree or a k-d tree and construct one partition tree $\syn_h$ with $k$ leaf nodes for each query template $h\leq L$. Each node of every $\syn_h$ stores the (updated) statistics and the associated (hyper-)rectangle of the corresponding $h$-th partitioning. The only difference now is that we do not store the samples in the leaf nodes of each tree. Instead, whenever we need access to the samples in a leaf node $u$, we run a reporting query with the corresponding hyper-rectangle $R_u$ in the range tree (or k-d tree). In this way, using only $O(m+L\cdot k)$ space, we have theoretical error guarantees for every different query that belongs in one of the supported query template. The update time increases by a factor of $L$, however, all update operations in a tree are extremely fast and they can be executed in parallel for different trees.
Furthermore, we note that ideally in our system we would like to know all query templates upfront so that the corresponding tree is ``ready'' when we get a query from a supported template. However, even if the templates are not known upfront, when we see a query from a new template we can construct a new partition tree using our efficient partitioning algorithms in roughly $O(k\cdot\polylog m)$ time. Then we start the catch-up phase only for this tree and start answering queries from this new template with error guarantees.
Finally, we notice that the user can give an overall memory constraint, and not one memory constraint for each different synopsis. Using the overall upper bound, our system can automatically decide and update the number of samples we store or the size of the partition trees that we maintain in order to satisfy the memory constraint.
}

\reviewtwo{
Second method: There is also a simpler, heuristic way to handle queries from different templates using only one partition tree \syn. Imagine that we construct a partition tree using the SUM aggregation function over the aggregation attribute $A$ and predicate attributes $c_1, \ldots, c_d$. If the user asks a query with a different type of aggregation function, say AVG or COUNT, we can still use the same tree to answer the query as long as we store and maintain the sum and the count in each node of the tree. If the user asks a query with a different aggregation attribute $B$ instead of $A$ there are two ways to handle it: i) We store and maintain statistics in \syn for all attributes including $B$ (we always assume constant number of attributes). Hence, we can still answer a query using the partition tree straightforwardly. ii) If we do not store and maintain statistics for all attributes, then we can perform stratified sampling using the strata and the samples in the leaf nodes of the \syn.
Finally, assume that the system encounters a new query having different predicate attributes. There are a few ways to handle it: i) Assume that the dynamic partition tree \syn we constructed at the beginning was constructed over all possible predicate attributes of the tuples. Recall that throughout our submission we always assume a constant number of attributes. We can always query such tree with any query range over any subset of predicate attributes and return an estimation with confidence intervals. The tree is not optimized strictly with respect to the predicate attributes of the query (as in the first method) however we expect the error to be low. ii) Simply apply uniform sampling using the samples $\samples$, or iii) re-partition the tree for the new predicate attributes.
%We conduct more experiments in this revision in Section~\ref{sec:experiments} using this simpler heuristic to handle dynamic query templates showing the error in each different case
}

\iffalse
\reviewtwo{
This new method we described here has the same theoretical error guarantees we had before with respect to the optimum partitioning over the exact query template.
Here, we describe a heuristic to support different query templates using only one partition tree.
We can still have confidence intervals but we do not have any guarantee on how far the confidence intervals are with respect to the optimum (shortest) confidence intervals we could get from an optimum partitioning.
Imagine that we have already constructed a partition tree \syn using the SUM aggregation function over an aggregation attribute $A$ and predicate attributes $c_1,\ldots, c_d$. If the user asks a query with a different aggregation function, say COUNT, we can still use the same tree \syn to answer it. We might not have the same theoretical guarantees but the error will be better comparing to simpler methods like random sampling or stratified sampling.
If the user asks a query with a different aggregation attribute $B$ instead of $A$ there are two ways to handle it: i) We store and maintain low-error statistics in \syn for all attributes including $B$. Hence, we can still answer a query using the partition tree straightforwardly. ii) If we do not store and maintain statistics for all attributes, then we can perform stratified sampling using the strata and the samples in the leaf nodes of the \syn.
Finally, the most challenging update is changing the predicate attributes. There are also two ways to handle it: Either apply uniform sampling using the samples $\samples$ or re-partition the tree for the new predicate attributes.}
\fi



%In Section~\ref{sec:experiments} we run eusing this simpler heuristic to handle dynamic query templates studying the error in each different case.

%If the user changes the aggregation attribute from $A$ to $B$, we can still use the same tree as long as we maintain the low-error statistics for $B$ in the nodes of the tree. If the system knew upfront that the user will ask queries using $B$ in the future, the statistics in the inner nodes of \syn would be updated for both $A$ and $B$. Hence, we could also answer a query with better error guarantees than other simpler methods. If we did not know the attribute $B$ upfront then we apply stratified sampling using as strata all the leaf nodes of the tree that are intersected or fully contained in the query predicate. Finally, if the predicate attributes are changed, this is indeed the most difficult case to handle. If should not construct a second partition tree, we just apply uniform sampling taking the samples from $S$ that belong in the query predicate.}

==> additionals.tex <==

In this section we propose new algorithms for constructing a partition over the samples items $\samples$. Our algorithms can be used in different scenarios: i) construct a partition the first time over $\samples$, ii) construct a new partition if the re-partition is needed after a number of updates in our dataset, and iii) check if repartition is needed after an insertion or deletion of an item, i.e., is there a partition with significantly less error than the current partition?
%In the end of this section we formally describe how Dynamic PASS decides when a re-partition/re-construction of $\PASStree$ is needed.

In~\cite{liang2021combining} the authors proposed algorithms for constructing near optimal partitions.
However, most their algorithms run in time roughly $O(km\log m)$. For the offline version of the problem their algorithm is very efficient since it is linear in both parameters $k, m$. Ideally, in the dynamic setting, we do not want the update procedure to depend linearly on $m$, i.e., the number of samples we store. Here we design data structures and algorithms that run the re-partition (or the check if there is a better partition) in only $O(k)$ time, ignoring $\polylog$ factors, which is near-optimal since we have $k$ buckets.

In order to achieve faster algorithms we propose new dynamic data structures for various sub-problems. Mainly, we propose an efficient dynamic data structures such that given a query rectangle, it returns (approximately) the maximum variance of a query completely inside the query rectangle. Using this data structure, we can achieve a very fast construction of $\PASStree$ in any dimension $d$.
For $d=1$ we manage to design a very efficient algorithm making an assumption on the aggregation values of the items. In particular we assume that the values of items are bounded by a polynomial on $N$, i.e. the total number of items in the full dataset. This is usually the case in real datasets so it is not a strong assumption and it is made in several papers~\cite{guha2006approximation} for constructing histograms with low error. %We notice that the assumption is not needed in higher dimensions.

We start by introducing some basic notation and by defining some basic notions. Then we describe our new dynamic data structures for finding maximum error queries.
We continue by presenting the partition algorithm for $d=1$ and the partition algorithm for any dimension $d>1$.
In the end of this section we show an algorithm to decide when re-partition is needed.


\subsection{Preliminaries}
The goal of \sys is to construct a dynamic partition tree $\PASStree$ such that the maximum error (confidence interval) of a query is minimized. Recall that the leaf nodes of $\PASStree$ define a partition over the samples $\samples$.
As we discussed in previous sections the number of samples $H$ (catch-up phase) is going to be much larger than the number of samples in $\samples$. In particular, the sampling rate of $H$ in the end of the catch-up phase is significantly higher than the sampling rate of $\samples$ we store in $\PASStree$. Hence we expect that the error (variance) of nodes in $U_2$ will be much lower comparing to the error of the nodes in $U_1$ for a query $q$. So we focus on finding a partition that minimizes the longest confidence interval of any possible query considering only the error from the leaf nodes that partially intersect the query.

As shown in~\cite{liang2021combining}, in order to find the query with the worst confidence interval in the partition defined by the leaf nodes of $\PASStree$, it is sufficient to consider only queries that lie completely inside the leaf nodes of $\PASStree$.
Indeed by considering only these queries we can still get a $\sqrt{k}$-approximation for COUNT and SUM queries over the optimum partition considering all queries. The approximation factor improves to $\sqrt{2}$ for $d=1$. For AVG queries the error of the optimum partition considering queries completely inside the leaf nodes is the same with the maximum error considering every possible query. So without loss of generality we solve the optimization problem of finding a partition that minimizes the maximum error considering only queries that lie completely inside the buckets of a partition.


%Static PASS~\cite{hellerstein2008quantitative} tries to find a tree structure such that its leaf nodes define a partition over the samples $\samples$ to (approximately) minimize the length of the longest confidence interval. Equivalently, in PASS they are trying to find a partition that minimizes the maximum error. The authors in~\cite{liang2021combining} argue that instead of looking over all possible queries to minimize the maximum error they focus on queries that lie completely inside one bucket. Indeed, the optimum partition considering only queries that lie completely inside a bucket has error at most $\sqrt{k}$ times more than the error over the optimum partition for COUNT/SUM queries. For AVG queries the error of the optimum partition considering queries completely inside buckets is the same with the maximum error considering every possible query.


%Similarly to~\cite{liang2021combining}, considering only queries completely inside a bucket gives a $\sqrt{k}$ approximation for COUNT/SUM queries and $1$-approximation (optimum) for AVG queries. For $1$D it gives a $\sqrt{2}$ approximation for COUNT/SUM queries.

Let $u$ be a leaf node of $\PASStree$ and let $q$ be a query completely inside $R_u$. In this case notice that $w_u=1$ for all types of queries.
From Section~\ref{sec:estimators}, recall that the variance of any COUNT or SUM query completely inside $R_u$ has a factor $\frac{N_u^2}{m_u^2}$. This factor is the same in all queries inside $u$ so without loss of generality we can skip it from the variance definition (considering queries inside $R_u$).
Furthermore, notice that the confidence interval of any query inside $R_u$ has a factor $\frac{1}{m_u}$ which is also the same. Hence, the problem of finding the query with the largest confidence interval in $u$ is equivalent with the problem of finding the query $q$ in $u$ that maximizes the following function.
If $q$ is a COUNT or SUM query:
$$\nu_s(q)=m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2,$$
and if $q$ is an AVG query:
$$\nu_s(q)=\frac{1}{|q|^2}\left[m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2\right].$$


In order to make sure that we return accurate estimators we require that each bucket contains a sufficiently large amount of samples, roughly $\Omega(\frac{1}{\alpha}\log m)$ samples, where $\alpha$ is the sampling rate of $\samples$.
%If that holds, it is known from~\cite{liang2021combining} that with high probability the ratio $\frac{N_u}{m_u}$ for any possible leaf node $u$ will be within a constant factor from the ratio $N/m$, so it will be almost the same for any bucket we construct.
Furthermore, we study queries that contain at least $\delta m$ samples from each bucket that they partially intersect, for a small parameter $\delta<1$. Otherwise a query does not include many samples and we are not be able to return an accurate estimator along with a provable confidence interval. We note that these assumptions were also made in~\cite{liang2020fast}.
%Finally, we define the following notation which is useful in the next subsections. For a rectangle $R$, let $\optVar(R)$ be the variance of the query with the maximum variance in $R$.

==> dpt_old.tex <==
However, if we do not allow a full pass over $\fullData$ at the first construction of $\PASStree$, or after the first re-partition, we do not have the exact statistics in every node of the new tree $\PASStree$. After the construction of the main structure of $\PASStree$ we start a \emph{catch-up phase} where Dynamic PASS gets samples (in the background) from $\fullData$ to improve the statistics in the nodes of $\PASStree$. Given a sample $s$ from the catch-up phase we visit $\PASStree$ from the root to the corresponding leaf node updating the estimations of the statistics (as shown in Section~\ref{sec:estimators}) in $O(\ell)$ time. Let $H$ be the samples we get in the catch-up phase. We note that we do not store any samples from $H$ in Dynamic PASS, instead we only use them to improve the estimators of the nodes in $\PASStree$.  Since the catch-up phase runs in the background (in a different thread) there is no need to have a small duration. It is important to mention that Dynamic PASS can still answer aggregation queries and handle updates as the catch-up phase is running.


Since we do not have the exact statistics of the nodes as in the static PASS, we expect that the error of Dynamic PASS will be worse.
However, the catch-up phase is running  repeatedly (until it finishes) in the background so $|H|>>|\samples|$. Hence, we expect that queries that partially intersect leaf nodes will still have the higher error (longer confidence intervals). By optimizing a partition over the query with the largest error (Section~\ref{sec:partAlg}) we expect that the worst error of Dynamic PASS will only be slightly worse than the worst error of Static PASS leading to very accurate estimators.





As we mentioned in the issue (3), it might be possible that the current partition $\PASStree$ is not good enough for the updated set of samples $\samples$. For example, there might not be many samples in a leaf node (bucket) so the estimations are not robust, or the maximum confidence interval (error) is too large in $\PASStree$. In Section~\ref{sec:re-partition}
we describe an algorithm to decide when Dynamic PASS needs to re-partition. If a re-partition is needed we need to construct the new $\PASStree$ very fast so that the system is ready to support new queries as soon as possible. The algorithms in~\cite{liang2021combining} to construct a new partition  tree run in roughly $O(km)$ time. Ideally in the dynamic setting we do not want to spend $\Omega(m)$ time to construct the tree. In Section~\ref{sec:partAlg} (using the results of Section~\ref{sec:updateVar}) we propose new novel dynamic data structures with $O(m)$ space that allow us to construct the new partition tree $\PASStree$ in time roughly $O(k)$, which is optimal if a new partition with $k$ buckets needs to be constructed.


\subsection{Catch-Up Optimization}
In order to make PASS dynamic we need to propose non-trivial solutions to multiple problems.
Some of the core problems we need to consider are the following: (1) How to maintain a set of random samples $\samples$ over insertions and deletions? (2) How can we return estimators with provable confidence intervals under updates? (3) What if the current partition tree $\PASStree$ is not good enough (high error) with respect to the current set of samples $\samples$? Do we need to re-construct $\PASStree$? (4) How can we construct a new partition tree efficiently (in time that doe not depend on $m$)? (5) How can we maintain the statistics in the nodes?

In Section~\ref{sec:estimators} we show how to extend the estimators and the confidence intervals of static PASS for the Dynamic PASS. In a high level, we use estimators over the old data in $\fullData$ and we use exact statistics over the new inserted or deleted items.
Before the first re-partition if we allow to make a full pass over $\fullData$ as we construct $\PASStree$, someone can update all the exact statistics of the nodes in $\PASStree$ over insertions and deletions. Indeed, given a new insertion $t$ we can update the exact estimators from the root to the leaf node $u$ such that $t.p\in R_u$. Similarly we can update the aggregation functions in the nodes when a deletion happens in $O(\ell)$ time. 

==> maxVarUpdates.tex <==
\subsection{Maximum variance under updates}
\label{sec:updateVar}


\mparagraph{Minimizing the error}
\stavros{TODO}
Static PASS~\cite{hellerstein2008quantitative} tries to find a tree structure such that its leaf nodes define a partition over the samples $\samples$ to (approximately) minimize the length of the longest confidence interval. Equivalently, in PASS they are trying to find a partition that minimizes the maximum error.
The authors in~\cite{liang2021combining} argue that instead of looking over all possible queries to minimize the maximum error they focus on queries that lie completely inside one bucket. Indeed, the optimum partition considering only queries that lie completely inside a bucket has error at most $\sqrt{k}$ times more than the error over the optimum partition for COUNT/SUM queries. For AVG queries the error of the optimum partition considering queries completely inside buckets is the same with the maximum error considering every possible query.

In dynamic PASS we have the same goal: minimize the length of the longest confidence interval. As we discussed in previous sections the number of samples $H$ (catch-up phase) is going to be much larger than the number of samples in $\samples$. In particular the sampling rate of the catch-up phase in the end of the catch-up phase is usually significantly higher than the sampling rate of samples we store in dynamic PASS. Hence we expect that the error (variance) of nodes in $U_2$ will be much lower comparing to the error of the nodes in $U_1$ for a query $q$. So we focus on finding a partition that minimizes the longest confidence interval of any possible query considering only the error from the leaf nodes that partially intersect the query.
Similarly to~\cite{liang2021combining}, considering only queries completely inside a bucket gives a $\sqrt{k}$ approximation for COUNT/SUM queries and $1$-approximation (optimum) for AVG queries. For $1$D it gives a $\sqrt{2}$ approximation for COUNT/SUM queries.

Notice that when we study a query $q$ completely inside a leaf node $u$ we only care about the variance $$V(q)=m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2$$ if $q$ is a  COUNT/SUM query, or $$V(q)=\frac{1}{|q|^2}\left[m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2\right]$$ if $q$ is an AVG query. This is true because the weight $w_u$ and the denominator $m_u$ in the confidence interval is the same for every query in $u$. Hence, we can only focus on the variance of queries in a node to find the one with the longest confidence interval. 
In order to make sure that we return accurate estimators we require that each bucket contains a sufficiently large amount of samples, roughly $\Omega(\frac{1}{\alpha}\log m)$ samples, where $\alpha$ is the sampling rate of $\samples$.
If that holds, it is known from~\cite{liang2021combining} that with high probability the ratio $\frac{N_u}{m_u}$ for any possible leaf node $u$ will be within a constant factor from the ratio $N/m$, so it will be almost the same for any bucket we construct.
Furthermore, we study queries that contain at least $\delta m$ samples from each bucket that they partially intersect, for a small parameter $\delta<1$. Otherwise a query does not include many samples and we are not be able to return an accurate estimator along with a reasonable confidence interval. We note that these assumptions were also made by the authors in the static PASS~\cite{liang2020fast}.
Finally, we define the following notation that is useful in the next sections. For a rectangle $R$, let $\optVar(R)$ be the variance of the query with the maximum variance in $R$.



An important procedure of our algorithms is to be able to find what is the maximum error of a query that lies completely in a leaf node. We explain how to do it for the queries COUNT, SUM, AVG.
In particular, we describe a stronger result: We construct a dynamic data structure over a set of samples $\samples$ with efficient update time such that given a query rectangle, it returns an approximation of the variance of the query with the maximum variance in the query rectangle.
This result leads to very efficient dynamic algorithms for checking the maximum variance and re-constructing a new partition, as we will see in the next section.
As the authors in~\cite{liang2021combining} we use the notation $\maxVar$ for this procedure, i.e., $\maxVar(R)$ returns an approximation of the maximum variance of a query (COUNT, SUM, or AVG) in a rectangle $R$.

\mparagraph{COUNT queries}
For COUNT queries it is known~\cite{liang2021combining} that the query with the maximum variance in a rectangle $R$ contains exactly $|R\cap P|/2$ samples.
Hence, we construct a dynamic range tree~\cite{} $T$ over $\samples$ with space $O(m\log^d m)$. $T$ can be constructed in $O(m\log^d m)$ time and can be updated in $O(\log^d m)$ time. Given a query rectangle $R$, we run a binary search using $T$ to find two rectangles that contain $|R_i|/2$ items. The query runs in $O(\log^d m)$ time.

\mparagraph{SUM queries}
In ~\cite{liang2021combining} the authors showed that given a rectangle $R$ we can find a $\frac{1}{4}$-approximation of the variance of the query with the maximum variance inside $R$ by doing the following simple procedure: Find two non-intersecting rectangles $R_1, R_2$ such that $R_1\cup R_2=R$, and $|R_1\cap P|=|R_2\cap P|=|R\cap P|/2$. Then, they compare $\sum_{t\in R_1\cap P}t.a^2$ with $\sum_{t\in R_2\cap P}t.a^2$ and they return the variance of the rectangle with the largest sum of squares. The variance of this rectangle is a $\frac{1}{4}$-approximation of the maximum variance in $R$.
Range trees work for any aggregation function so we can also use them to compute the sum of the values squared in a rectangle or the variance of a rectangle.
Hence, we can use a dynamic range tree as we had in the COUNT case returning a $\frac{1}{4}$-approximation of the maximum variance. Notice that in this case we use the range tree for all procedures: i) finding two rectangles with the same number of samples ii) computing the sum of their squared values, and iii) compute the variance of a rectangle. This data structure has exactly the same complexities as in the COUNT case.

%As the authors in~\cite{liang2021combining} showed, we need $O(\log^{d-1} m)$ time to find an approximation of the maximum variance query in a bucket, using a range tree. Using a dynamic range tree~\cite{} for every bucket, we can achieve $O(\log^d m)$ update time for any insertion/deletion of a sample, and we can get a $1/4$-approximation of the maximum variance query.

\mparagraph{AVG queries}
The authors in~\cite{liang2021combining} proposed a way in the offline case to get an approximation on the maximum variance AVG query in a set of samples. In particular, their algorithm returns a $\frac{1}{4}$-approximation in $1$D, $\frac{1}{8}$-approximation in $2$D and $\frac{\delta^{1-1/d}}{2}$-approximation for $d>3$ and it runs in time superlinear . 
Unfortunately, their data structures cannot be efficiently extended to the dynamic case we are interested in (is not known how to achieve $\polylog m$ update time).
Here we propose a new dynamic data structure for finding an approximation of the maximum variance AVG query in a query rectangle efficiently. The new data structure we propose does not only handle updates efficiently, unlike the data structures in~\cite{liang2021combining}, but it also improves the approximation factor for any dimension $d$.
%All their algorithms can be made dynamic using dynamic data structures. Here, we briefly discuss their data structures and how they can be made dynamic. In the end we propose a new approximation dynamic algorithm with better approximation factor that works in any constant dimension $d$.




%In $1$D they use a search binary tree that stores the sum of squares of $\delta m$ consecutive samples in the leafs. In the inner nodes it stores the maximum such value that appear in the subtree of the inner node. The tree can be constructed in $O(m\log m)$ time and has $O(m)$ space. Given an interval the tree structure can return a $\frac{1}{4}$-approximation in $O(\log m)$ time. When we insert or delete a sample $t\in P$ we need to update the sums of the leafs that $t$ participates in and udpate the maximum values in the inner nodes. Notice that any sample participates in at most $O(\delta m)$ leaf nodes, hence this tree can be updated in $O(\delta m + \log m)$ time. We can easily modify this tree to return a $\frac{1}{8}$-approximation in $O(\log \frac{1}{\delta})$ time, with update time $O(\frac{1}{\delta})$. In $2$D, they only use a range tree, so we can use a dynamic range tree~\cite{} and handle insertion or deletions. This data structure has $O(m\log^d m)$ space, can be updated in $O(\log^{d} m)$ time, and returns a $\frac{1}{8}$-approximation of the maximum variance in a rectangle in $O(\log^{d+2} m)$ time. In higher dimensions, they propose a modified k-d tree where each leaf contains $\delta m$ samples. They return the rectangle that corresponds to the leaf node with the maximum sum of squares of the values, as the query with the maximum variance. Given a query rectangle, this procedure finds a $\frac{\delta^{1-1/d}}{2}$-approximation of the maximum variance in $O(\min\{\frac{1}{\delta}\log^d m, m\log m\})$ time. This k-d tree can be made dynamic~\cite{} having roughly the same complexities.

For a set of samples $\samples$ we construct a dynamic range tree $T'$. We also initialize an empty dynamic data structure $T$ that stores weighted rectangles. Given a query rectangle $R$, it returns the rectangle with the highest weight that lies completely inside $R$. For example $T$ can be a dynamic range tree in $2d$ dimensions storing each rectangle as a $2d$ point by creating a point from its two main opposite corners.
Notice that every $d$-th level node $u$ of $T'$ corresponds to a rectangle $R_u$.
If $|R_u\cap P|\leq \delta m$ then we add $R_u$ in $T$ with weight $S(R_u)=\sum_{t\in R_u\cap P}t.a^2$. If $\delta m\leq |R_u\cap P|\leq 2\delta m$ we split $R_u$ into two rectangles $R_{u_1}, R_{u_2}$ such that $R_{u_1}\cup R_{u_2}=R_u$ and $|R_{u_1}\cap P|=|R_{u_2}\cap P|=|R_u\cap P|/2$. We add $R_{u_1}, R_{u_2}$ in $T$ with weights $S(R_{u_1})=\sum_{t\in R_{u_1}\cap P}t.a^2$, $S(R_{u_2})=\sum_{t\in R_{u_2}\cap P}t.a^2$.
The tree $T'$ can be constructed in $O(m\log^d m)$ time and it has $O(m\log^d m)$ space. In $T$ we might insert $O(m\log^d m)$ rectangles so it has $O(m\log^{3d} m)$ space and can be constructed in $O(m\log^{3d} m)$ time. For any insertion or deletion of a sample in $\samples$, $T'$ can be updated in $O(\log^d m)$ time by modifying at most $O(\log^d m)$ nodes. For each modified node we update accordingly the corresponding rectangle in $T$ in $O(\log^{2d}m)$ time. Furthermore, after an update we traverse the $d$-th level of the tree from the updated leaf nodes to their roots inserting or removing rectangles from $T$ accordingly. In the full version of the paper we describe an amortized way to update $T$ efficiently that can be made worst case update by standard techniques~\cite{}.
Overall our data structure can be constructed in $O(\log^{3d} m)$ time, has $O(\log^{3d} m)$ space and can be updated in $O(\log^{3d+1} m)$ time.


%and a modified dynamic range tree $T$ as follows. Let $u$ be a node of $T$ and $w_1, w_2$ are its two children. If $|R_{w_1}\cap P|=|R_{w_2}\cap P|<\delta m$ and $|R_u\cap P|>\delta m$ then we stop the execution of $T$ in this branch of the tree and we create the two nodes $w_1, w_2$ containing exactly $\delta m$ samples by expanding their corresponding rectangles to contain more samples. Notice that a sample might belong in both $w_1, w_2$. In this way we have a dynamic range tree where in every leaf node (in any level of the range tree) it contains exactly $\delta m$ samples. It is not necessary to construct $T$ as a separate data structure from $T'$ since we can easily run all procedures by slightly changing the procedures on $T'$ with a $\polylog m$ overhead. However, we refer to $T$ as a separate data structure for simplicity. For each leaf node $u$ (over all levels) of $T$ we store $S.u=\sum_{t\in R_u\cap P}t.a^2$. Then for each inner node $u$ in the last ($d$-th) level of $T$ we store and maintain the maximum $S_w$ value among the leaf nodes $w$ with root the node $u$, i.e., $M.u=\max_{w\in leaf(u)}S_w$, where $leaf(u)$ is the set of leaf nodes of the tree rooted at node $u$. Our data structure (both trees $T, T'$) is constructed in $O(m\log^d m)$ time, has $O(m\log^d m)$ space, and can be updated in $O(\log^d m)$ time.

Given a query rectangle $R$ such that $R\cap P>2\delta m$ (as the authors in~\cite{liang2021combining} assume) we show how to return an approximation of the maximum variance query  efficiently.
We search $T$ using the query rectangle $R$ and we get a set of $O(\log^{2d} m)$ canonical nodes that contain all rectangles completely inside $R$. From the canonical subsets we get the rectangle $q'$ inside rectangle $R$ with the largest weight.
If $|q'\cap P|<\delta m$ then 
using $T'$ we run binary search over all dimensions until we find an expansion of $q'$ that contains exactly $\delta m$ samples. This can be done in $O(\log^{d+1} m)$ time. Without loss of generality assume that $q'$ is this rectangle. Using $T'$ we measure the variance of $q'$ in $R$ in $O(\log^d m)$. In the end we return the variance of $q'$ as the approximation of the maximum variance AVG query in the query rectangle $R$. The query procedure takes $O(\log^{2d} m)$ time.


%If $u$ is a leaf node of $T$ visited by the query procedure that partially intersects $R$ we do the following. From the definition $|R_u\cap P|=\delta m$ so $|R_u\cap R\cap P|\leq \delta m$. Assume that indeed the rectangle $R_u\cap R$ contains less than $\delta m$ samples. In this case we want to make sure that we create a rectangle containing exactly $\delta m$ samples inside $R$. Using $T'$ we run binary search over all dimensions until we find an expansion of the rectangle $R_u\cap R$ that contains exactly $\delta m$ samples inside $R$. Let $R_u'$ be this expanded rectangle. Using $T'$ we also get $\sum_{t\in R_u'\cap P} t.a^2$. In the end, without loss of generality the query procedure in $T$ finds a set of $O(\log^d m)$ (possibly overlapping) rectangles that cover $R$ and each of the rectangles containing $\delta m$ samples. Using the pre-computed values $M.u$ along with the values $\sum_{t\in R_u'\cap P} t.a^2$ we computed in the query procedure we return the rectangle with the largest sum of squared values. Let $q'$ be that rectangle. Using $T'$ we measure the variance of $q'$ in $O(\log^d m)$ time. In the end we return the variance of $q'$ as the approximation of the maximum variance AVG query in the query rectangle $R$. The query procedure takes $O(\log^{2d} m)$ time since there are $O(\log^d m)$ rectangles (leaf nodes of $T'$) that partially intersect $R$ and for each of them we need $O(\log^d m)$ to find new rectangles fully inside $R$ that contain $\delta m$ samples.

Next, we show that the variance we return is a good approximation of the real maximum variance in rectangle $R$.
\begin{lemma}
It holds that $V(q')\geq \frac{1}{4\log^d m}\optVar(R)$.
\end{lemma}
\begin{proof}
Let $q$ be the AVG query (a rectangle) with the maximum variance in $R$. It is known from~\cite{liang2021combining} that $q$ contains at most $2\delta m$ and at least $\delta m$ samples.
Since $|R\cap P|\geq 2\delta m$ we have that $$|R\cap P|\sum_{t\in q'\cap P}t.a^2-\left(\sum_{t\in q'\cap P}t.a\right)^2\geq \frac{|R\cap P|}{2}\sum_{t\in q'\cap P}t.a^2,$$
following from Lemma A.2 in~\cite{liang2021combining}.
Next, notice that a query procedure on $T'$ with the query range $q$ would give a set of $\log^d m$ canonical rectangles that cover $q$ where each of them contains at most $2\delta m$ samples. We note that for each of these canonical rectangles in $T'$ there are at most two rectangles in $T$ containing the same items. Let $X$ be the set of rectangles in $T$ corresponding to the canonical rectangles in $T'$. From its definition it holds that $|X|\leq 2\log^d m$. All of these rectangles in $X$ lie completely inside $R$ so the query procedure will consider them to find the rectangle with the largest weight.
Hence it holds that 
$$\sum_{t\in q'\cap P}t.a^2\geq \max_{x\in X}\sum_{t\in x\cap P} t.a^2\geq \frac{1}{2\log^d m}\sum_{t\in q\cap P}t.a^2.$$ Overall we have,
\begin{align*}
    V(q')&=\frac{1}{|q'\cap P|^2}\left[|R\cap P|\sum_{t\in q'\cap P}t.a^2-\left(\sum_{t\in q'\cap P}t.a\right)^2\right]\\
    &\geq \frac{1}{|q'\cap P|^2}\frac{|R\cap P|}{2}\sum_{t\in q'\cap P}t.a^2\\
    &\geq \frac{1}{|q'\cap P|^2}\frac{1}{4\log^d m}|R\cap P|\sum_{t\in q\cap P}t.a^2\\
    &\geq \frac{|q\cap P|^2}{|q'\cap P|^2}\frac{1}{4\log^d m}\frac{1}{|q\cap P|^2}\left[|R\cap P|\sum_{t\in q\cap P}t.a^2-\left(\sum_{t\in q\cap P}t.a\right)^2\right]\\
    &\geq \frac{1}{4\log^d m}\mathcal{V}(R)
\end{align*}
\end{proof}
In the full version we show that if $d=1$ we can modify the data structure so that it gives an approximation factor $4$ while having slightly better complexities with respect to the exponents of the $\log m$ factor.

Overall, given a set $P$ of $m$ points in $d$ dimensions we can construct a data structure of space $O(m\cdot \polylog (m))$ in $O(m\cdot \polylog (m))$ time with update time $O(\polylog (m))$ such that given a query rectangle it finds an approximation of the maximum variance COUNT, SUM or AVG query inside $R$ in $O(\polylog (m))$ time.

%We propose a new algorithm to find an approximation of the maximum variance in any constant dimension $d$. Instead of constructing a k-d tree we construct a dynamic range tree~\cite{} where each leaf node contains $\delta m$ samples. It might be possible that a sample belongs in two leaf nodes that are siblings in order to make sure that each leaf node has $\delta m$ samples. For each leaf node $u$ in the $d$-th level of the range tree we store and maintain the sum of squares of the values of the items in $u$. Then we store the leaf nodes in a max-heap with respect to the sum of squares we computed. This data structure can be constructed in $O(m\log^d m)$ time and it has $O(m\log^d m)$ space. For an insertion or deletion of a sample $p$ the range tree can be updated in $O(\log^d m)$ time~\cite{}, so at most $O(\log^d n)$ nodes of the tree might be modified or inserted. For each modified/inserted node we compute its sum and we update the max-heap. The max-heap can be updated in $O(\log n)$ time so in total the update time of our data structure is $O(\log^{d+1} n)$. In order to find an approximation of the maximum variance query we return the rectangle that corresponds to the leaf node with the largest sum of squares, i.e., the leaf node at the root of the max-heap. Such a rectangle contains $\delta m$ samples with the largest sum of squares over all other $d$-level leaf nodes. Let $q^*$ be the rectangle that corresponds to the query with the maximum variance. A standard range tree can find a partition of $q^*$ with $O(\log^d m)$ canonical nodes/rectangles. Since $|q^*|\leq 2\delta m$ it is not possible that a canonical node will contain any of the leaf nodes of our modified range tree. Hence, for each canonical node $u$ of $q^*$ in the standard range tree we can always find one leaf node in our modified range tree that completely covers $u$. Following the proof in~\cite{liang2021combining} we show that our algorithm returns a $\frac{1}{4\log^d m}$-approximation of the maximum variance query.

==> partition-old.tex <==
In order to achieve faster algorithms we propose new dynamic data structures for various sub-problems. Mainly, we propose an efficient dynamic data structures such that given a query rectangle, it returns (approximately) the maximum variance of a query completely inside the query rectangle. Using this data structure, we can achieve a very fast construction of $\PASStree$ in any dimension $d$.
For $d=1$ we manage to design a very efficient algorithm making an assumption on the aggregation values of the items. In particular we assume that the values of items are bounded by a polynomial on $N$, i.e. the total number of items in the full dataset. This is usually the case in real datasets so it is not a strong assumption and it is made in several papers~\cite{guha2006approximation} for constructing histograms with low error. %We notice that the assumption is not needed in higher dimensions.

We start by introducing some basic notation and by defining some basic notions. Then we describe our new dynamic data structures for finding maximum error queries.
We continue by presenting the partition algorithm for $d=1$ and the partition algorithm for any dimension $d>1$.
In the end of this section we show an algorithm to decide when re-partition is needed.





Let $u$ be a leaf node of $\PASStree$ and let $q$ be a query completely inside $R_u$. In this case notice that $w_u=1$ for all types of queries.
From Section~\ref{sec:estimators}, recall that the variance of any COUNT or SUM query completely inside $R_u$ has a factor $\frac{N_u^2}{m_u^2}$. This factor is the same in all queries inside $u$ so without loss of generality we can skip it from the variance definition (considering queries inside $R_u$).
Furthermore, notice that the confidence interval of any query inside $R_u$ has a factor $\frac{1}{m_u}$ which is also the same. Hence, the problem of finding the query with the largest confidence interval in $u$ is equivalent to the problem of finding the query $q$ in $u$ that maximizes the following function.
If $q$ is a COUNT or SUM query:
$V(q)=m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2$
and if $q$ is an AVG query:
$V(q)=\frac{1}{|q|^2}\left[m_u\sum_{t\in q}t.a^2-\left(\sum_{t\in q}t.a\right)^2\right]$.


In order to make sure that we return accurate estimators we require that each bucket contains a sufficiently large amount of samples, roughly $\Omega(\frac{1}{\alpha}\log m)$ samples, where $\alpha$ is the sampling rate of $\samples$.
%If that holds, it is known from~\cite{liang2021combining} that with high probability the ratio $\frac{N_u}{m_u}$ for any possible leaf node $u$ will be within a constant factor from the ratio $N/m$, so it will be almost the same for any bucket we construct.
Furthermore, we study queries that contain at least $\delta m$ samples from each bucket that they partially intersect, for a small parameter $\delta<1$. Otherwise a query does not contain many samples in a leaf node and we are not be able to return an accurate estimator along with a provable confidence interval. We note that these assumptions were also made by the authors in the static PASS~\cite{liang2020fast}.
Finally, we define $\optVar(R)$ to be the variance of the query with the maximum variance in $R$.
